Causal Intervention for Fairness in Multi-behavior Recommendation

Recommender systems usually learn user interests from various user behaviors, including clicks and post-click behaviors (e.g., like and favorite). However, these behaviors inevitably exhibit popularity bias, leading to some unfairness issues: 1) for items with similar quality, more popular ones get more exposure; and 2) even worse the popular items with lower popularity might receive more exposure. Existing work on mitigating popularity bias blindly eliminates the bias and usually ignores the effect of item quality. We argue that the relationships between different user behaviors (e.g., conversion rate) actually reflect the item quality. Therefore, to handle the unfairness issues, we propose to mitigate the popularity bias by considering multiple user behaviors. In this work, we examine causal relationships behind the interaction generation procedure in multi-behavior recommendation. Specifically, we find that: 1) item popularity is a confounder between the exposed items and users' post-click interactions, leading to the first unfairness; and 2) some hidden confounders (e.g., the reputation of item producers) affect both item popularity and quality, resulting in the second unfairness. To alleviate these confounding issues, we propose a causal framework to estimate the causal effect, which leverages backdoor adjustment to block the backdoor paths caused by the confounders. In the inference stage, we remove the negative effect of popularity and utilize the good effect of quality for recommendation. Experiments on two real-world datasets validate the effectiveness of our proposed framework, which enhances fairness without sacrificing recommendation accuracy.

==> 2_method_v1.tex <==
\section{Methodology}
% In this section, we firstly analyze the two kinds of fairness and propose to estimate the two unfairness by two metrics. Then we analyze the impact of item popularity on multi-behavior recommendation from a causal view. In the end, we propose a multi-behavior debiasing framework that mitigates the bad effect of popularity bias through causal interventions.


In this section, we first formulate two fairness problems by considering multiple user behaviors, and then we discover the reasons for unfairness from a causal view. Lastly, we introduce the MBD framework to mitigate the unfairness problem via two interventions.
% we first define two metrics to estimate the two kinds of unfairness in multi-behavior recommendation. Then we analyze the impact of item popularity on multi-behavior recommendation from a causal view to better understand the reasons of unfairness. In the end, we propose a multi-behavior debiasing framework that mitigates the bad effect of popularity bias through causal interventions.

\subsection{Fairness in Multi-behavior Recommendation}\label{sec:fairness_formulation}

%%%%%

% the definition of the first fairness: for items the same quality, more popular items get more exposure. 
% to quantify exposure. 我们参考XXX 用公式XX来计算exposure.
% to quantify quality, 我们借鉴某个文章，用ratioXXX来估计quality. 实验在XXX上也证明了item quality和like/click ratio的线性相关关系。具体地，XXX解释。
% Finally, the first fairness is to pursue minimizing 公式5.

% worse still, the definition of the second fairness: for items the lower quality, a higher popularity leads to more exposure. 
% 我们参考文章28 用XXX来衡量第二种fairness，具体地，第二种fairness is to minimize 公式6。


%%%%%
% To better analyze the two kinds of unfairness introduced in the previous section, we need to define and quantify them in the recommendation results.

% different from PDA: 优化目标、多行为、quality。 
% In recommender systems, popularity not only affects the exposure of an item~\cite{zhang2021causal}, but also correlates with other factors, such as the quality of the item. 
% Previous work does not focus on the influence of popularity with other factors in optimizing the popularity bias problem, as well as the recommendation fairness problem. 
Previous work either removes popularity bias (\eg MACR~\cite{wei2021model}) or leverages popularity via causal inference to achieve better accuracy (\eg PDA~\cite{zhang2021causal}). 
% Existing work tends to reduce the impact of popularity bias or making use of popularity for better accuracy. 
However, they only focus on the accuracy regarding one kind of user behavior, ignoring the relations between multiple user behaviors and the unfairness caused by popularity bias.
Different from MACR~\cite{wei2021model} and PDA~\cite{zhang2021causal}, we propose utilizing multiple user behaviors to measure item quality, and mitigate the unfairness issues by explicitly modeling the relations between popularity and quality.
% In this paper, we focus on the relations between popularity and item quality in multi-behavior recommendation, and then find two kinds of unfairness problems.

% In the previous section, we introduce two kinds of unfairness in multi-behavior recommendation.

\vspace{5pt}

\noindent\textbf{$\bullet$ Calculation of unfairness.} Since not all the datasets have the item quality score, it is difficult to estimate it directly. In this work, we propose to use the item's post-click conversion ratio to make an approximation. 
Previous research~\cite{lalmas2015promoting} and our experiments both demonstrate the positive correlation between the item quality and post-click conversion ratio. 
We conduct experiments on the popular Zhihu\footnote{https://github.com/THUIR/ZhihuRec-Dataset.} dataset, where the collection number of articles strongly reflects the item quality. Figure~\ref{fig:quality_zhihu} clearly presents the positive correlation between collection number and the post-click conversion ratio. In this figure, the value of Spearman's correlation coefficient~\cite{abdullah1990robust,hauke2011comparison} is $0.8361$ and the $p$-value is $4.4e^{-6}$, which also prove the rationality of approximating quality by the post-click conversion ratio. 

\begin{figure}[t]
% \vspace{-2.5cm}
    \centering
    \includegraphics[width=.35\textwidth]{figures_multi/zhihu_quality.pdf} 
    \vspace{-5pt}
    \caption{Collections of articles \wrt post-click conversion ratio from reads to likes.}
    \label{fig:quality_zhihu}
    \vspace{-10pt}
\end{figure}

To calculate the exposure for each item in the ranking list, we refer to the position bias defined in the discounted cumulative gain~\cite{jarvelin2002cumulated}. Formally, the exposure of item $i$ can be obtain by:
\begin{equation}\label{equ:exposure}
\left \{
\begin{aligned}
    & v_{j} = \frac{1}{log_{2}(1 + j)}, \\
    & exp(i|P_{i}) = \sum_{j = 1}^{N} P_{i, j} * v_{j},
\end{aligned}
\right .
\end{equation}
where $v_j$ denotes the exposure probability of the $j$-th item in the ranking list, and $P_{i,j}$ is the probability of item $i$ recommended at the position of $j$. 

To evaluate the first fairness, we argue that the items with similar quality should receive similar exposure. As such, we divide items into groups based on item quality, and then split each group into subgroups according to different popularity. Thus, we can measure the exposure difference between these subgroups to evaluate the first fairness. Formally, we estimate the exposure of a subgroup $G$ by averaging the item-level exposure:
\begin{equation}\label{equ:exposure_g}
    Exp(G) = \frac{1}{|G|}\sum_{i \in G} exp(i|P_{i}).
\end{equation}

Specifically, we first estimate the average quality of groups, and then use the exposure/quality disparity between different groups to evaluate the second unfairness. Formally,
\begin{equation}\label{eq:disparity_general}
\left \{
\begin{aligned}
&Ratio(G) = \frac{1}{|G|} \sum_{i \in G} r_{i}, \\
&D(G_1, G_2) = \left|\frac{Exp(G_1)}{Ratio(G_1)} - \frac{Exp(G_2)}{Ratio(G_2)}\right|,
\end{aligned}
\right .
\end{equation}
where $r_i$ is the post-click conversion ratio of item $i$, and $D_{l}(G_1, G_2)$ describes the unfairness between the groups $G_1$ and $G_2$. A small disparity $D_{l}$ implies that items receive the exposure proportional to their quality.


\noindent\textbf{$\bullet$ First Fairness.} The first kind of unfairness is that for items with same quality, more popular ones usually get more exposure. 
% To evaluate the fairness, the exposure and the quality of items are two variables to be quantified. 
To evaluate this unfairness, we need to quantify the item's exposure probability.
Thereafter, given two subgroups $G_1$ and $G_2$ with similar quality but different clicks (\ie different popularity), the first fairness aims to minimize the exposure disparity $D_r$ between them:
\begin{equation}\label{eq:disparity1}
    D_{r}(G_1, G_2) = |Exp(G_1) - Exp(G_2)|.
\end{equation}

\noindent\textbf{$\bullet$ Second Fairness} The second unfairness is that for items with the lower quality, a higher popularity may lead to more exposure. Following previous work~\cite{morik2020controlling}, we introduce a fairness criteria that relates exposure to item quality. 
Specifically, we first estimate the average quality of groups, and then use the exposure/quality disparity between different groups to evaluate the second unfairness. Formally,
\begin{equation}\label{eq:disparity2}
D_{l}(G_1, G_2) = \left|\frac{Exp(G_1)}{Ratio(G_1)} - \frac{Exp(G_2)}{Ratio(G_2)}\right|,
\end{equation}
where $r_i$ is the post-click conversion ratio of item $i$, and $D_{l}(G_1, G_2)$ describes the unfairness between the groups $G_1$ and $G_2$. A small disparity $D_{l}$ implies that items receive the exposure proportional to their quality.

\subsection{Causal View of Unfairness}\label{ssec:causal graph}
The causal graph is a directed acyclic graph $G = \{V, E\}$, where $V$ denotes a set of variables, and $E$ represents the causal relations among variables~\cite{pearl2009causality}. 
To analyze the reasons for the two kinds of unfairness, we abstract a causal graph in Figure \ref{fig:rec_graph}(a) that describes the causal relations between item popularity, quality, and multiple user behaviors. We explain the causal graph as follows:
\begin{itemize}[leftmargin=*]
    % \item Node $U$ represents the user node, \eg user profile or history feature that is used for representing a user. 
    % \item Node $I$ represents the item node. We assume a user can only interact (\eg click, post-click) with the items that have been exposed to him/her, thus $I$ denotes the exposed item. 
    \item $U$ and $I$ denote users and items, respectively. We assume that users can only interact with the items exposed to them, and thus $I$ represents the exposed items. 
    % \item Node $C$ represents the click probability, indicating whether the user has clicked the exposed item. 
    \item $C$ is the click probability of the user clicking the exposed item. 
    \item $L$ is the post-click probability, indicating whether the user has a post-click behavior (\eg favourite and like) on the exposed item.
    \item $Z$ represents the item popularity, which is estimated by item's received interactions.
    \item $Q$ represents the item quality, which is a hidden variable and cannot be easily quantified. As discussed in Section~\ref{sec:fairness_formulation}, we propose to approximately estimate it by the conversion ratio from clicks to post-click behaviors. If the clicked item has better quality, users should have a higher probability of liking it.
    \item $T$ represents some unobserved variables, such as the reputation and scale of item producers.
    \item $\{U, I\}\rightarrow C$: the click probability is affected by the user and exposed items. 
    \item $Z\rightarrow I$: item popularity affects the exposure of items. The recommendation models are usually trained on long-tailed data. Therefore, they tend to give popular items more exposure~\cite{germano2019few}. 
    \item $\{U, I\}\rightarrow L$: the user and exposed items determine the probability of post-click behaviors.
    \item $C\rightarrow L$: only clicked items can have post-click behaviors.
    \item $\{Z, Q\}\rightarrow L$: item popularity and quality affect the probability of post-click behaviors. Meanwhile popularity influences users' post-behaviors because of the users' herd mentality (\aka conformity)~\cite{zhang2021causal}.
    \item $Z \leftarrow T \rightarrow Q$: T affects both $Z$ and $Q$, causing the confounding effect between the two variables. For example, item producer reputation can affect the popularity of items because users tend to consume items with famous brands or well-reputed producers, making such items more likely to become popular.
    Besides, the quality of items is often affected by item producer reputation or the business scale of the producer.
    
    % denotes that the quality of items are often affected by some unobserved variables (\eg item producer reputation, scale of the producer).
    % \item $T \rightarrow Z$ denotes some unobserved variables (\eg item producer reputation) can affect the popularity of items. For example, users tend to consume items with famous brands or well-reputed producer, which will make such items more likely become popular.
\end{itemize}

\noindent\textbf{$\bullet$ Reason for two unfairness issues.} With the help of the causal graph in Figure \ref{fig:rec_graph}(a), we can explore the true reasons for the two kinds of unfairness. Firstly, we find that item popularity $Z$ is a confounder between $I$ and $L$, causing the first backdoor path $I\leftarrow Z\rightarrow L$. The backdoor path results in that for the same quality items, more popular ones are more likely to be exposed to the user via $Z\rightarrow I$ and receive higher post-click probabilities by $Z\rightarrow L$ due to users' herd mentality, which reflects the first kind of unfairness~\cite{zhang2021causal}. 
Moreover, $T$ and $Z$ are confounders between $Q$ and $L$, causing the second backdoor path $Q\leftarrow T\rightarrow Z \rightarrow L$. Thus, item quality is correlated with popularity because of unobserved confounder $T$ via $Q\leftarrow T\rightarrow Z$. Then some low-quality items might correlate with high popularity, which will bring more exposure to such popular items. This explains the second unfairness.

To summarize, two backdoor paths cause two kinds of unfairness in multi-behavior recommendation. To alleviate the unfairness, we need to cut off these two backdoor paths for removing the bad impact of such confounders.



\subsection{MBD Framework}\label{sec:MBD_framework}

In this work, we propose a MBD framework that leverages \textit{backdoor adjustment}~\cite{pearl2009causality} to cut off the backdoor paths and remove the bad effect caused by the confounders. Specifically, as shown in Figure \ref{fig:rec_graph}(b), we perform the intervention $do(I=i)$ by controlling the observed variable $Z$ to block the backdoor path $I \leftarrow Z \rightarrow L$. 
However, for the second backdoor path $Q \leftarrow T \rightarrow Z \rightarrow L$, $Q$ and $T$ are unobserved variables that make the backdoor adjustment infeasible. 
Thanks to the post-click conversion ratio that reflects the item quality (see Section \ref{sec:fairness_formulation}), we propose to use it for the approximation of item quality $Q$. 
Instead of controlling the unobserved $T$, we can achieve the intervention on $Q$ by controlling $Z$, which also blocks the second backdoor path. 
Besides, considering the critical impact of item quality in the recommendation, we estimate the post-click probability via $P(L|U, do(I), do(Q))$.

We denote the causal graph shown in Figure \ref{fig:rec_graph}(a) as $G$ and the intervened causal graph shown in Figure \ref{fig:rec_graph}(b) as $G'$, and then we will derive the following expression on $G$:
\begin{subequations}
\label{equ:P_do_IQ}
\begin{align}
&P(L|U,do(I),do(Q))=P_{G^\prime}(L| U,I,Q) \notag \\
                &=\sum_{Z}\sum_{C}{P_{G^\prime}(L| U,I,Q,Z,C)P_{G^\prime}(C|U,I,Q)}P_{G^\prime}(Z| U,I,Q) \\
                &=\sum_{Z}\sum_{C}{P_{G^\prime}(L|U,I,Q,Z,C)P_{G^\prime}(C|U,I)}P_{G^\prime}(Z) \\
                &=\sum_{Z}P_{G^\prime}(L|U,I,Q,Z,C=1)P_{G^\prime}(C=1|U,I)P_{G^\prime}(Z)+ \sum_{Z}P_{G^\prime}(L|U,I,Q,Z,C=0)P_{G^\prime}(C=0|U,I)P_{G^\prime}(Z) \\
                &\approx\sum_{Z}P_{G^\prime}(L|U,I,Q,Z,C=1)P_{G^\prime}(C=1| U,I)P_{G^\prime}(Z)\\
                &=\sum_{Z}P(L|U,I,Q,Z,C=1)P(C=1| U,I)P(Z),
\end{align}
\end{subequations}
where $P_{G'}(\cdot)$ denotes the probability function estimated by $G'$. The derivation of Equation \ref{equ:P_do_IQ} is as follows: 
% to be changed and completed
\begin{itemize}[leftmargin=*]
    \item (5a) and (5c) are due to \textit{Bayes' theorem};
    \item (5b) is because of the $do$-calculus on $I$ and $Q$. The first backdoor path $I\leftarrow Z\rightarrow L$ is blocked by $do(I=i)$, which mitigates the first unfairness. The second backdoor path $Q\leftarrow T\rightarrow Z \rightarrow L$ is blocked by $do(Q=r_i)$, which mitigates the second unfairness. Thus, $P_{G^\prime}(Z|U,I,Q)$ can be deduced as $P_{G^\prime}(Z)$. $P_{G^\prime}(C|U,I,Q)$ changes into $P_{G^\prime}(C|U,I)$ because $C$ is independent from $Q$. The user cannot know the item quality $Q$ before clicking the item;
    % \item (1c) is because of \textit{Bayes' theorem}. The user has two choices: click or not click the item, which corresponds to $C=1$ and $C=0$;
    \item (5d) is because we do not consider the non-clicked data;
    \item (5e) is because of the same prior of $U, I, Z, Q$ on two graphs. $\{U, I, Z, Q\}\rightarrow L$ will not be changed by cutting off two paths $Z\rightarrow I$ and $T\rightarrow Q$.
\end{itemize}

\begin{figure}[t]
% \vspace{-2.5cm}
    \centering
    \includegraphics[width=.5\textwidth]{figures_multi/workflow2.pdf} 
    % \vspace{-5pt}
    \caption{The implementation of MBD. The CTR function and CVR function are the user-item matching functions $f_{c}$ and $f_{l}$, respectively. The purple arrows indicate that the item popularity $Z$ is used in the training stage but removed from the inference stage.}
    \label{fig:framework}
    \vspace{-10pt}
\end{figure}

Next, we need to consider how to estimate $P(L|U,do(I),do(Q))$ from the data. From the derived expression (5e), we need to firstly estimate $P(L|U,I,Q,Z,C=1)$ and $P(C=1|U,I)$, respectively, and then estimate $\sum_{Z}P(L|U,I,Q,Z,C=1)P(C=1|U,I)P(Z)$ to get the prediction score. The estimations are as follows:


\vspace{+5pt}
\noindent \textbf{1) Estimating $P(C=1| U,I)$.} 
% This is the conditional probability that given user $U=u$, item $I=i$, how likely the user will click the item (\ie the click-through ratio (CTR)). 
This is the conditional click probability between users and items (\ie the click-through ratio (CTR)~\cite{richardson2007predicting}).
% todo: (CTR) 后面加一个reference，有CTR介绍的就行
To parameterize $P(c=1|u,i)$, we use $f_c$ to represent the user-item matching function for clicks, which can be realized by any user-item matching model (\eg Matrix Factorization (MF)~\cite{koren2009matrix}). % todo: （MF）后面加一个ref
Hence, the probability can be calculated as:

\begin{equation}\label{equ:f_ctr}
    p_{ctr} = P(c=1|u,i) = \sigma(f_{c}(u, i)),
\end{equation}
where $\sigma$ is the sigmoid function to normalize the matching score between 0 and 1. 
% We calculate the CTR loss by Cross-Entropy loss on the historical click data $\mathcal{D}$ that is also composed of the sampled user's unclicked items as negative samples:
We instantiate the CTR loss by the cross-entropy loss on the historical click data $\mathcal{D}$, which
consists of users' sampled unclicked items as negative samples:

\begin{equation} \label{equ:loss_ctr}
    L_{ctr}  = \sum_{(u, i)\in \mathcal{D}} - \hat{y}_clog(p_{ctr}) \\- (1-\hat{y}_c)log(1-p_{ctr})),
\end{equation}
where $\hat{y}_c\in\{0,1\}$ is the user click feedback on items. In addition, we apply $L_2$ regularization but omit it for brevity.


\vspace{+5pt}
\noindent \textbf{2) Estimating $P(L|U,I,Q,Z,C=1)$.} This conditional probability estimates that given $U=u$, $I=i$, item quality $Q=r_i$ and item popularity $Z=z_{i}$, how likely the user will have post-click behavior on the clicked item (\ie the post-click conversion ratio (CVR)). Same with CTR,
% , how to design the function is an important question. We
% we use the design method of \cite{zhang2021causal} for reference, the conditional probability can be calculated as
we calculate this conditional probability by:

\begin{equation}
    p_{cvr} = P(l=1|u,i,r_{i},z_{i},c=1)=\sigma(f_{l}(u,i))r_{i}^{\gamma_r}z_{i}^{\gamma_z},
\end{equation}
where $\sigma$ is the sigmoid function, and $f_l$ can be implemented by any user-item matching model. The hyper parameter $\gamma_z$ is used to smooth the item popularity and $\gamma_r$ is used to control the influence of the like/click ratio of item $i$, \ie $r_i = \frac{n_{i,l}}{n_{i,c}}$, where $n_{i,l}$ and $n_{i,c}$ are the number of post-click behaviors and clicks, respectively. %on post-click probability. 
% \begin{equation}\label{equ:ratio}
%     r_i = \frac{n_{i,l}}{n_{i,c}}.
% \end{equation}
% As Equation~\eqref{equ:ratio}, the value of $r_i$ can be estimated by the ratio of item's received post-clicks $n_{i,l}$ on clicks $n_{i,c}$. 
We normalize the ratio $r$ and the popularity $z$ by the min-max normalization~\cite{al2006data} to make sure that they are the same scale. Next, we can estimate the click through\&conversion ratio (CTCVR) as:
%  by $p_{ctcvr} = p_{ctr}*p_{cvr}$, which can be calculated as:

\begin{equation}\label{equ:f_ctcvr}
\begin{aligned}
p_{ctcvr} &= P(l=1|u,i,r_{i},z_{i},c=1)*P(c=1|u,i)\\
            &=\sigma(f_l(u,i))r_{i}^{\gamma_r} z_{i}^{\gamma_z}\sigma(f_{c}(u,i)).  
\end{aligned}
\end{equation}
We calculate the CTCVR loss by the cross-entropy loss:

\begin{equation}\label{equ:loss_ctcvr}
     L_{ctcvr} = \sum_{(u, i)\in \mathcal{D}_l} - \hat{y_l}log(p_{ctcvr})\\ -(1-\hat{y}_l)log(1-p_{ctcvr}),
\end{equation}
where $\hat{y}_l\in\{0,1\}$ denotes whether the user has post-click behavior on the item, and $\mathcal{D}_l$ collects the historical post-click data. 
% todo: check 是不是like
The overall loss $\mathcal{L}$ consists of two loss terms from the CTR and CTCVR predictions: 

\begin{equation}\label{equ:finalloss}
    \mathcal{L} = L_{ctr} + L_{ctcvr}.
\end{equation}


\vspace{+5pt}
\noindent \textbf{3) Estimating $\sum_{Z}P(L|U,I,Q,Z,C=1)P(C=1| U,I)P(Z)$.} At last, with the help of above two steps, we can estimate the interventional probability $P(L|U,do(I),do(Q))$ as follows:
\begin{subequations}\small
\label{equ:to be named}
\begin{align}\small
&P(L|U,do(I), do(Q)) \notag\\
                &=\sum_{Z}{P(L|U,I,Q,Z,C=1)P(C=1|U,I)P(Z)}  \\
                &=\sum_{Z}\sigma(f_l(u,i))r_{i}^{\gamma_r} z_{i}^{\gamma_z}\sigma(f_{c}(u,i))p(Z)   \\
                &=\sigma(f_{c}(u,i))\sigma(f_l(u,i))r_{i}^{\gamma_r}\sum_{Z} z_{i}^{\gamma_z}p(Z)   \\
                &=\sigma(f_{c}(u,i))\sigma(f_l(u,i))r_{i}^{\gamma_r}E(Z^{\gamma_z}),
\end{align}
\end{subequations}
where $E(Z^{\gamma_z})$ is the expectation of $Z^{\gamma_z}$ which is a constant and does not change the recommendation results. As Figure \ref{fig:framework} shows, we use Equation~\eqref{equ:finalloss} to train the matching functions $f_{c}(u,i) $ and $f_l(u,i)$, and model the influence of the popularity $z_i$ and quality $r_i$ on $L$ at the training stage. Thereafter, we remove the influence of the confounder $z_i$ to alleviate the two unfairness issues, \ie estimating the deconfounded prediction $s$ to rank item candidates:
\begin{equation}\label{equ:score_inference}
    s(u, i, r_{i}) = \sigma(f_{c}(u,i))\sigma(f_l(u,i))r_{i}^{\gamma_r}.
\end{equation}

% \subsection{Comparison with $P(L|U,I,Q)$}
% To see the difference between the traditional correlation-based method and the MBD with interventions, we analyze the different factors between these two methods.
% The traditional method can be transformed as follows:

% \begin{subequations}
% \label{equ:tradition}\small
% \begin{align}\footnotesize
% &P(L|U,I,Q) \notag\\
%                 &=\sum_{Z}\sum_{C}{P(L| U,I,Q,Z,C)P(C|U,I,Q)}P(Z|U,I,Q) \\
%                 &=\sum_{Z}P(L|U,I,Q,Z,C=1)P(C=1|U,I)P(Z|I,Q)+ \\
%                 &\sum_{Z}P(L|U,I,Q,Z,C=0)P(C=0|U,I)P(Z|I,Q) \notag \\
%                 &\approx\sum_{Z}P(L|U,I,Q,Z,C=1)P(C=1| U,I)P(Z|I,Q)\\
%                 &\propto\sum_{Z}P(L|U,I,Q,Z,C=1)P(C=1| U,I)P(I,Q|Z)P(Z)\\
%                 &=\sum_{Z}P(L|U,I,Q,Z,C=1)P(C=1| U,I)P(I|Z)P(Q|Z)P(Z),
% \end{align}
% \end{subequations}
% where (11a) is because of Bayes' theorem; (11b) is because of Bayes' theorem and $U$ is independent of $Z$; (11c) and (11d) is because of Bayes' theorem and $I$ is independent of $Q$ and (11e) is because of the independence between $Q$ and $I$. 

% Through the comparison of the two methods, we find that $P(C|U, I, Q)$ has two different terms: $P(I|Z)$ and $P(Q|Z)$, which are the reasons of the two kinds of unfairness. For example, if we assume that $I=i$ is a popular item, $P(I=i|Z=z_{i})$ will probably be a significant value due to the amplification of exposure by recommender systems. That is the reason for the first unfairness. Due to the influence of unobserved variables $T$, some low-quality items might get high popularity. Therefore, $P(Q=r_{i}|Z=z_{i})$ might be a large value for some low-quality items, which will give them a high score than they deserve, and leads to the second unfairness. Such two factors are eliminated by interventions in our proposed MBD framework, and thus $P(L|U, do(I), do(Q))$ is necessary to mitigate the two unfairness and learn the unbiased user interests from the data with popularity bias.
% \vspace{-5pt}

% Suppose $I=i$ is a popular item, $P(C|U, I=i, Z=m_i^t)$ is a large value since $m_i^t$ is large, which means the term has a large contribution to the prediction score. $P(I=i | Z=m_i^t)$ is also a large value due to the popularity bias in the exposure mechanism. Multiplying the two terms further enlarges the score of $i$, which gives $i$ a higher score than it deserves. As a result, the popularity bias is improperly amplified. This comparison further justifies the rationality and necessity of $P(C|do(U,I))$ for learning user interests reliably.
\vspace{-10pt}
\begin{algorithm}[]
	\caption{MBD}
	\LinesNumbered
	\label{algo}
	\KwIn{dataset $\mathcal{D}=\{(u,i,z_{i},r_{i})\}$; hyper-parameter $\gamma_{r}, \gamma_{z}$; CTR and CTR models: $f_{c}$, $f_{l}$;}
	\While{stop condition is not reached}{
	    \If {training}{
            Calculate $p_{ctr}$ by Equation~\eqref{equ:f_ctr}\;
            Get CTR loss $L_{ctr}$ by Equation~\eqref{equ:loss_ctr}\;
	        Calculate $p_{ctcvr}$ by Equation~\eqref{equ:f_ctcvr}\;
	        Get CTCVR loss $L_{ctcvr}$ by Equation~\eqref{equ:loss_ctcvr}\;
	        $\mathcal{L} = L_{ctr} + L_{ctcvr}$\;
	        Optimize $\mathcal{L}$ to update $f_{c}$ and $f_{l}$\;
        }
        \If {validating or testing}{
            Recommend the items using deconfounded score $s(u,i,r_i)=\sigma(f_{c}(u,i))\sigma(f_l(u,i))r_{i}^{\gamma_r}$\;
        }
	}
\end{algorithm}
\vspace{-5pt}





 




==> 2_primary_experiment_and_knowledge.tex <==
\section{Primary knowledge}
% In this section, we would like to introduce the symbols that we used for recommendation. And then show that item popularity trends are drift with time goes to show that it's desirable to introduce some bias in recommendation.
We use uppercase character (\eg $U$) to denote a random variable and lowercase character (\eg $u$) to denote its specific value. We use characters in calligraphic font (\eg $\mathcal{U}$) to represent the sample space of the corresponding random variable, and use $P(\cdot)$ to represent probability distribution of a random variable. 

% \paragraph{Problem formulation.} 
Let $\mathcal{D}$ denote the historical data, which is sequentially collected through $T$ stages, \ie $\mathcal{D} = \{\mathcal{D}_1 \cup \cdots \cup \mathcal{D}_T\}$; $\mathcal{U}=\{u_1 , \dots, u_{|\mathcal{U}|}\}$ and $\mathcal{I}=\{i_1 , \dots, i_{{|\mathcal{I}|}}\}$ denote all users and items, respectively. 
%The target of recommender system is to learn the user preference over items from historical user behaviors. 
Through learning on historical data, the recommender system is expected to capture user preference and serves well for the next stage $T+1$. That is, it aims to obtain high recommendation accuracy on $\mathcal{D}_{T+1}$. 
%That is, estimating the probability that a user clicks a item in the future stage $T+1$. 
%In our setting, we investigate the effect of item popularity.% which is a term defined over a set of interactions. 
In this work, we are interested in the factor of item popularity, defining the \textit{local popularity} of item $i$ on the stage $t$ as: 
%Formally, for each stage t, we defined the popularity of item $i$ over $\mathcal{D_t}$ as
%  \begin{equation}\label{eq:pop_define}\small
%      m_{i}^{t} = \frac{D_{i}^{t}}{\sum_{j\in \mathcal{I}} D_{j}^{t}},
%  \end{equation}
 \begin{equation}\label{eq:pop_define}\small
     m_{i}^{t} = D_{i}^{t} / \sum_{j\in \mathcal{I}} D_{j}^{t},
 \end{equation}
where $D_{i}^{t}$ denotes the number of observed interactions for item $i$ in $\mathcal{D}_{t}$. We can similarly define the global popularity of an item $m_i$ based on its interaction frequency in $\mathcal{D}$, but we think the local popularity has a larger impact on the system's exposure mechanism and user decision, since the system is usually periodically retrained and the most recent data has the largest impact. 

%Aiming to investigate the popularity bias, we introduce an extra variable $Z$ to represents item popularity. Note that $Z$ is a variable, and  each $m_{i}^{t}$, is the instance of $Z$ on the interactions containing the item $i$ in the stage $t$.    



% Accordingly, we can calculate the item popularity at stage $t$, which is termed as $m_i^t$. Aiming to investigate the popularity bias, we introduce an extra variable: $Z$, which represents to what extent the recommendation strategy was influenced when an interaction was collected. That is to say, each instance of $Z$ represents a recommendation strategy \wrt item popularity. In particular, we can abstract the instance as a mapping that describes how likely the recommendation strategy will recommendation an item with popularity of $m_i$.

%It' hard to be observed in data directly.
%that represents the recommendation strategy which is determined by system and influence by history popularity. It's a hidden variable and hard to observed in data; % $Z$ that represents history item popularity; 
%$M$ represents the current popularity of one item. In particular, let $D_i$ denotes the number of interactions for item $i$ on $\mathcal{D}$, then the popularity for one item can be computed as following: 
%By representing the user, item, and click as three random variables, $U$, $I$, $C$, most existing recommender systems estimates $P(C|U, I)$ over the historical data by optimizing a recommendation loss, assuming taking BPR Loss~\cite{}, it is formulated as:
% 
% \begin{equation}\label{eq:bpr}
%     \min \sum_{(u, i^{+}/i^{-}, c) \in \mathcal{D}/\mathcal{D}^-} -log( \sigma(P(c |u, i^{+}) - P(c |u, i^{-})) ),
% \end{equation}
% 
% \begin{equation}
%     \min \sum_{(u, i, c) \in \mathcal{D}/\mathcal{D}^-} l(c, P(c|u, i)),
% \end{equation}
% \begin{equation}
% \min \sum_{(u, i, c) \in \mathcal{D}/\mathcal{D}^-} log(sigmoid(P(c^+ | u,i) - P(c^+ | u,i) ))
% \end{equation}
% 
% where $\mathcal{D}^-$ denotes randomly selected negative samples and $\sigma(\cdot)$ is the sigmoid activation function. Note that we omit the parameters of the probability distribution $P(C|U, I)$ for briefness, which are indeed the parameters of the recommender model. 
% 
%We focus on implicit recommendation, which is deeply influenced by popularity bias. Using $\mathcal{D}$ represents a dataset. And we split $\mathcal{D}$ into $T$ chunks along timestamp, the t-th chunk denotes as a stage $\mathcal{D}_t$. The last sub-dataset $\mathcal{D}_{T}$ is used to valuation and testing, and others are treated as training set. The goal is to estimate the probability that a user click a item. Let $\mathcal{U}=\{u_1 , \dots, u_{|\mathcal{U}|}\}$ and $\mathcal{I}=\{i_1 , \dots, i_{{|\mathcal{I}|}}\}$ denote the users and items set respectively. In figure~\ref{fig:rec_causal_pre_now}, $U$ and $I$, $C$ are variables that represent user, item and click probability, where $C$ is a binary variable. Then $(u,i,c)$ is a instance of $(U,I,C)$, and an element of $D$ if $c=1$. The Standard Collaborative Filtering use two sets of embedding that represent user/item to fit with $P(C|U,I)$. Because usually we only focus on $C=1$ and $C$ is binary, without special remark, we use $P(C|U,I)$ to represent $P(C=1|U,I)$. Besides above variables, we introduce $Z$ and $M$, where both of them are related to popularity. $Z$ represents a distribution of item popularity that can called history popularity or system-side popularity, it will influence how to recommend items. $M$ is the current popularity of one item, which can be compute as following: for one instance $(u,i,c)$, the corresponding instance of $M$ is:
%In our setting, we introduce two extra random variables: $Z$ is a hidden variable to represent what extent history popularity influences recommendation strategy. It' hard to be observed in data directly.
%that represents the recommendation strategy which is determined by system and influence by history popularity. It's a hidden variable and hard to observed in data; % $Z$ that represents history item popularity; 
%$M$ represents the current popularity of one item. In particular, let $D_i$ denotes the number of interactions for item $i$ on $\mathcal{D}$, then the popularity for one item can be computed as following: 
%popularity is a random variable that can be compute as following: 
% for item $i$, %instance $(u,i,c)$, the corresponding instance of $M$ is:
% the corresponding popularity is:
%  \begin{equation}\label{eq:pop_define}
%      m_i = \frac{1 + D_{i} }{ {|\mathcal{I}|}+ \sum_{j\in \mathcal{I}} D_{j} }
%  \end{equation}
% where $|\mathcal{I}|$ represent the total number of item. We extra add one interaction to each item to avoid the zeros appearing.   %$M$ is related to the mapping of $Z$ on $I$. 
 
 

% \subsection{Problem and Notation}
%  We focus on implicit recommendation, which is deeply influenced by popularity bias. Let $\mathbb{U} = \{u_0,\dots,u_{m-1}\}$ and $\mathbb{I} = \{i_0,\dots,u_{n-1}\}$ denote users set and items set respectively, where $m$ and $n$ are the counts of unique users and items. The $U,I,Z$ in figure~\ref{fig:rec_causal_pre_now} are variables, for which $(U,I,Z)= (u,i,z) $ is a instance, in which $(u,i)$ is usually treat as an observed interaction. Assume that each interaction has a corresponding timestamp denoted as $tt$ that represents the happening time. The popularity $z$ is not directly observed, we compute it as following:
%  \begin{equation} \label{eq:pop}
%     \begin{split}
%         &z = [z_0 , \dots, z_k , \dots, z_{n-1}] \\
%         &where, \\
%         &z_k = z_{i_k }= \frac{1 + \#interactions\, of\,i^{th}\,item }{n + \#interactions \,of \,all\, items}
%     \end{split}
% \end{equation}
% where '\#xxx' denotes 'the count of xxx'. Here We take the Z-normalization to normalize the popularity distribution. 




% \subsection{Desired popularity bias}
\paragraph{Popularity drift.} 
Intuitively, item popularity is dynamic and changes over time, meaning that the impact of popularity bias could also be dynamic. To quantify the popularity drift, 
%Considering that item popularity drifts over time~\cite{MostRecent}, it is necessary to quantify the change of item popularity (\ie popularity drift) to facilitate the study of popularity bias. 
%To achieve the target, 
we define a metric named \textit{Drift of Popularity} (DP) to measure the drift between two stages.
First, we represent each stage $t$ as a probability distribution over items: $\big[m_{1}^{t},\dots,m_{|\mathcal{I}|}^{t}\big]$, where each entry denotes an item's frequency in the stage. 
Then, we use the Jensen-Shannon Divergence (JSD)~\cite{js-range} to measure the similarity between two stages: 
%Considering that item popularity can be treated as a probability distribution over items, we define DP based on Jensen-Shannon Divergence (JSD)~\cite{js-range}, which is widely used to measure the similarity between two probability distributions. Formally:
\begin{equation}\small
    \begin{aligned}
    DP(t,s) = JSD\left(
        \big[m_{1}^{t},\dots,m_{|\mathcal{I}|}^{t}\big],
        \big[m_{1}^{s},\dots,m_{|\mathcal{I}|}^{s}\big]
    \right),
\end{aligned}
\end{equation}
% \begin{align}
%     DP(t,s) = JSD\left(
%         \big[m_{1}^{t},\dots,m_{|\mathcal{I}|}^{t}\big],
%         \big[m_{1}^{s},\dots,m_{|\mathcal{I}|}^{s}\big]
%     \right),
% \end{align}
where $t$ and $s$ are the two stages.
%; $m_i^{t}$ and $m_i^{s}$ represent the corresponding popularity of item $i$. 
Similar to JSD, the range of DP is $[0,log(2)]$, and a higher value indicates a larger popularity drift. 
%Item popularity will drift with time goes by, from the data perspective, popular items will be different in the different stage. To better predict the user's interaction, the popularity drift can be introduced in prediction. The popularity that will drift into is the desired popularity. To quantify the popularity drift between two stages, we define a metric named \textit{Drift of Popularity}(DP) based on Jensen-Shannon Divergence(JSD)~\cite{js-range}. JSD is used to measure the similarity between two probability distributions, and its value drops in $[0,log(2)]$~\cite{js-range}, a higher value means the more differences between the two distribution, and $JSD=0$ means the two distribution are the same. Then the DP can be defined as:
% $$DP(k,l) = JSD([m_{1}^{k},\dots,m_{|\mathcal{I}|}^{k}], [m_{1}^{l},\dots,m_{|\mathcal{I}|}^{l}])$$
% where $k,l$ denote stage $k$ and $l$, $m_i^{k}$ represent the item popularity of i in stage $k$, and $[m_{1}^{k},\dots,m_{|\mathcal{I}|}^{k}]$ can be treated a probability distributions regarding item popularity. 
%And we take Laplace Smoothing~\cite{Laplace-smothing} when computing item popularity to smooth $m$ to avoid zeros appearing. If the item popularity doesn't drift in two stage, the DP will be 0, otherwise, will be great than 0.
% Since JSD cannot process inputs with zeros, Laplace Smoothing~\cite{Laplace-smothing} is applied to item popularity in the calculation of DP.

Figure~\ref{fig:drit_showing}(a) shows the DP value of two successive stages, \ie $DP(t,t+1)$ where $t$ iterates from 1 to 9, on three real-world datasets (details in Section~\ref{exp:setting}). We can see that the popularity drift obviously exists in all three datasets, and different datasets exhibit different levels of popularity drift. 
Figure~\ref{fig:drit_showing}(b) shows the DP value of the first and present stage, \ie $DP(1,t)$, which measures the accumulated popularity drift. 
We can see a clear increasing trend, indicating that the longer the time interval is, the large popularity drift the data exhibits. 
%We then conduct a quantitative analysis of the popularity drift in the historical data. In particular, we calculate $DP(t,t+1)$, which reflects the popularity drift between adjacent stages; and $DP(1,t)$, which represents the popularity drift as compared to the first stage. 
%For explicitly showing the popularity drift, we split datasets to 10 stages, then we compute $DV(t,t+1)$ and $DV(1,t)$, where $t={1,\dots,9}$ represent different stages, to show the differences. 
%Figure~\ref{fig:drit_showing} shows the DP measure on three representative recommendation datasets (see Section~\ref{sec:dataset} for details). (1) From Figure~\ref{fig:drit_showing}(a), we can find that the popularity drift obviously exists in all the datasets, and different datasets have different levels of popularity drift. (2) From Figure~\ref{fig:drit_showing}(b), we can see that stages with longer interval exhibit larger popularity drift.
%
These results reveal that popularity bias and its impact also change with time. The popularity bias in the future stage differs from that of past stages. If we set the target of model generalization as pursuing high accuracy on the next stage data $\mathcal{D}_{T+1}$\footnote{To our knowledge, many industrial practitioners on recommender systems use the next stage data for model evaluation.}, then a viable way is to predict popularity trend and inject it into the recommendations.  
%change along time since due to the connection to item popularity. 
%Furthermore, the popularity bias in the future testing stage will also be different from the training stages. As such, endowing the recommender model with future popularity bias will improve the recommendation accuracy. 

%The results are shown in Figure~\ref{fig:drit_showing}. We can find:(1) for all the datasets, the popularity drift exists, and different datasets have different levels of popularity drift.  (2) If two stages have greater time interval, there are greater popularity drifts.
%These result tell us the item popularity will change, the popular item in the previous stage is not the one that we desired in the future. So, the desired popularity bias,\eg future popularity,  should be introduced. 

%item的popularity会随着时间drift, 反应在数据上就是不同阶段的pop items会不一样，为了能更好的预测下一阶段D_{T+1}的用户行为，就应该把pop drift考虑进来
%To show that it is necessary to introduce some extra popularity bias, we try to exhibit the desired popularity bias is always drifting. We think that the distribution of the frequency of interactions can be treated as the desired popularity bias to lift the recommendation accuracy. So we can realize the goal by showing the drift of the distribution of popularity in data. We define a metric $DV$ based on Jensen-shannon divergence, as following:
% $$ DV(k,l) = JS([m_1^{k} ,\dots, m_{{|\mathcal{I}|}}^k ] ,[m_1^{l} ,\dots, m_{{|\mathcal{I}|}}^l]) $$
% where $k$ and $l$ represent different stage $k$ and $l$, and $JS(\cdot)$ denotes the Jensen-shannon divergence, which is usually used to measure the difference between two distribution.

% For explicitly showing, we split datasets to 10 stages, then we compute $DV(t,t+1)$ and $DV(0,t)$, where $t={1,\dots,9}$ to represent different stage, to show the differences. The results are shown in Figure~\ref{fig:drit_showing}. We can find:(1) for all the datasets,  (2) The more far distance two sub-datsets are, the more difference of popularity they have. These result tell us the desired popularity will changed, the popularity in the previous dataset is not the one that we desired in the future. So, extral popularity bias should be introduced. 

%We show that it is necessary to introduce some extra popularity bias by exhibiting the the desired popularity will drift with times going. To show the drifts, two metric are introduced, they are $DV$ and $DR$, where $DV$ is used to show the distribution of popularity drifting between two instances of $Z$, and $DR$ is used to show the drifting of ranking generated by the popularity. $DV$ is defined as:
% $$ DV(k,l) = JS(z^k,z^l) $$
% where $z^k $ and $z^l $ represent two distributions of popularity, and $JS(\cdot)$ denotes the Jensen-shannon divergence, which is usually used to metric the difference between two distribution. $DR(k,l)$ is the overlapping rate of two lists sorted by the two distribution of popularity in the top $L$ with different weights. 

% For explicitly showing, we split datasets to 10 periods, we compute $DV(t,t-1), DR(t,t-1) $ and $DV(0,t), DR(0,t) $, where $t={1,2,\dots}$, to show that difference of the popularity that desired. The results are showing in figure~\ref{fig:drit_showing}.

% To show the existence of popularity, we split the dataset to some chunks along time line, each chunk correspond to one time period. And then we show the difference between two neighbouring periods. To show the difference, we respectively exhibit the drift of popularity value (popularity distribution drift), and the drift of ranking sorted by popularity. Regarding popularity values drifting, we take Jensen-Shannon divergence as the metric, which is usually used to metric the distance of two distribution,
%  \begin{equation}
%      Drift\_V (P_i,P_j)  = JS(P_i,P_j)
%  \end{equation}
%  $Drift\_V \in [0,log2]$ get zero only when there are not values drifting, i.e., $P_i = P_j$. We take popularity as a distribution. 
%  Then, we design a metric based on the overlapping of two list in top k positions to metric the drift about ranking: First, we sort the items by the popularity
%  with decreasing in descending order for period i and period i-1. 
%   \begin{equation}
%      rank_i = argsort(P_i);
%      rank_j = argsort(P_j) 
%  \end{equation}
% Then we count the overlapping items rates in different top k\%, 2k\%,..., n k\% between the two sorted list, denote them as $R_1^(ij),...,R_n^(ij)$. Then the metric is :
%  \begin{equation}
%      Drift\_R(P_i,P_j) = \sum_{k=1}^{n-1} \frac{R_k}{2^k} + \frac{R_n}{2^{n-1}} 
%  \end{equation}
%  $Drift\_R \ in [0,1] $ gets 0 only when $rank_i$ is same to $rank_j$ in the top nk\% of the lists. In Figure\ref{fig:drit_showing}, We show $Drift\_V_i = Drift\_V(P_i,P_{i-1})$  and $Drift\_V_i = Drift\_R(P_i,P_{i-1})$. We can find that different datasets have different degrees of popularity drifting. From $Drift\_V_i0$.

\begin{figure}
    \centering
    % \includegraphics[width=0.5\textwidth]{figures/drift_showing.pdf}
    \subfigure[$DP(t,t+1)$]{\includegraphics[width=0.23\textwidth]{figures/drift_neibor_type.pdf}}
    \subfigure[$DP(1,t)$]{\includegraphics[width=0.23\textwidth]{figures/drift_ref1_type.pdf}}
    \vspace{-15pt}
    %\caption{Item popularity distribution changes over time measured by JS divergence between different stages: (a) between t-th and $(t+1)$-th period, (b) between 1-th and t-th period.}
    \caption{Popularity drift between: (a) two successive stages $DP(t, t+1)$; (b) the first and present stage  $DP(1, t)$.}
    \vspace{-13pt}
    \label{fig:drit_showing}
\end{figure}

==> 3_method_v1.tex <==
\section{Methodology}
%In this section, we first analyze introduce the causal view of interaction generation process (Section~\ref{ssec:causal graph}), then elaborate the proposed PDA framework (Section~\ref{ssec:PD} and~\ref{ssec:PDA}) followed by an in-depth interpretation of the proposed PDA, compared with correlation based methods.
% In this section, we first analyze the reason of popularity bias amplification from a causal view (Section~\ref{ssec:causal graph}), then elaborate the proposed PDA framework (Section~\ref{ssec:PD} and~\ref{ssec:PDA}) followed by an in-depth interpretation of the proposed PDA.
We first analyze the impact of item popularity on recommendation from a fundamental view of causality. Then we present our PDA framework that eliminates the bad effect of popularity bias on training and intervenes the inference stage with desired bias. Lastly, we present in-depth analyses of our method.


\subsection{Causal View of Recommendation}\label{ssec:causal graph}
Figure \ref{fig:rec_graph}(b) shows the causal graph that accounts for item popularity in affecting recommendation. By definition, 
% \subsubsection{Causal graph}
%Causal model is used to descibe the logics of how the data is generated, in which causal graph is used to describe the causal relations between variables. 
%A causal graph can be described as a directed acyclic graph $G = \{V,E\}$, where $V$ is a set of nodes and $E$ is a set of directed edges. 
causal graph~\cite{pearl2009causality} is a directed acyclic graph where a node denotes a variable and an edge denotes a causal relation between two nodes~\cite{pearl2009causality}.
It is widely used to describe the process of data generation, which can guide the design of predictive models. Next, we explain the rationality of this causal graph.

\begin{itemize}[leftmargin=*]
    \item Node $U$ represents the user node, \eg user profile or history feature that is used for representing a user. 
    \item Node $I$ represents the item node. We assume a user can only interact with (\eg click) the items that have been exposed to him/her, thus $I$ denotes the exposed item. 
    \item Node $C$ represents the interaction label, indicating whether the user has chosen/consumed the exposed item.
    \item Node $Z$ represents the item popularity, which can be seen as a hidden variable since it is usually not explicitly modeled by traditional methods (\eg \cite{mf,lightgcn} form predictions with Figure \ref{fig:rec_graph}(a)). But it has a large impact on the recommendation. 
    \item Edges $\{U, I, Z\} \rightarrow C$ denote that an interaction label $C$ is determined by the three factors: user $U$, item $I$, and the item's popularity $Z$. Traditional methods only consider $\{U, I\}\rightarrow C$ which is easy to explain: the matching between user interest and item property determines whether a user consumes an item. Here we intentionally add a cause node $Z$ for capturing user conformity --- many users have the herd mentality and tend to follow the majority to consume popular items~\cite{conformity,DICE}. Thus, whether there is an interaction is the combined effect of $U, I$ and $Z$. 
    \item Edge $Z\rightarrow I$ denotes that item popularity affects the exposure of items. This phenomenon has been verified on many recommender models, which are shown to favor popular items after training on biased data~\cite{Himan-thesis}. 
    %Popular items are more likely to be exposed to users, since they take more proportion in the training data an
\end{itemize}

From this causal graph, we find that item popularity $Z$ is a confounder that affects both exposed items $I$ and observed interactions $C$. This results in two causal paths starting from $Z$ that affect the observed interactions: $Z\rightarrow C$ and $Z\rightarrow I\rightarrow C$. The first path is combined with user-item matching to capture the user conformity effect, which is as expected. In contrast, the second path means that item popularity increases the exposure likelihood of popular items, making the observed interactions consist of popular items more. Such effect causes bias amplification, which should be avoided since an authentic recommender model should estimate user preference reliably and is immune to the exposure mechanism.

In the above text, we have explained the causal graph from the view of data generation. In fact, it also makes sense to interpret it from the view of model prediction. Here, we denote $U$ and $I$ as user embedding and item embedding, respectively, and traditional models apply inner product~\cite{mf,lightgcn} or neural network~\cite{ncf} above them for prediction (\ie Figure \ref{fig:rec_graph}(a)). Item popularity $Z$ is not explicitly considered in most models, however, it indeed affects the learning of item embedding. For example, it increases the vector length of popular items, making inner product models score popular items high for every user~\cite{DICE}. Such effect justifies the edge $Z\rightarrow I$, which exerts a negative impact to learn real user interest. 

To sum up, regardless of which explanation for the causal graph, $Z\rightarrow I$ causes the bad effect and should be eliminated in formulating the predictive model. 
%and an edge represents the causal relation between the end nodes.
%Causal graph is widely used to describe the data generation process, \ie how the value of a node is affected by its father nodes~\cite{pearl2009causality}. 
%Such as showing in Figure~\ref{fig:rec_causal_pre_now}, $V=\{U,I,Z,M,C\}$ and $ E=\{U\rightarrow C, I\rightarrow C \dots \}$. Each node represents a variable. Each directed edge represents a causality that the source node causes the target node, usually the source is called father node and the target is called child node, and the source is a direct cause of the target. If one variable has one direct path, which consists of a series of directed edges in the same direction, to another variable, then the variable is a cause of the another. And specially, if a variable is a common cause of other two variables, then the variable is called confounder~\cite{pearl_primer,pearl2009causality} of the other two variables. For example, $Z$ is a confounder of $I$ and $M$. For each variable $X$, denotes its total fathers as $PA_X$, then $X$ can be generated by a function $f_X(PA_X)$, which describe how the $PA_X$ influence X. Such as $C$ and its fathers $U,I,M$, we use the $f_C (U,I,M)$ to represent the mechanism that how $U,I,M$ influence $C$.
%

%We abstract the generation process of interactions as the causal graph in the Figure~\ref{fig:rec_graph}(b). In the graph, $U$ represents user, $I$ represents exposed or recommended item, and $C$ is used to represent interaction event, such as Click. $Z$ represent item popularity.  $(U,I) \rightarrow C$ represent the user-item matching cause the interacting, which can be think as the true interest of $U$ to $I$. $Z \rightarrow I $ represent the $Z$ cause $I$, in particular, $Z$ will affect which item to be exposed. Such as if $Z$ is high, some group items, that manifest as more popularity in the dataset. Meanwhile, $Z$ will also cause $C$ by the path $Z\rightarrow C$, \ie itempopularity will directly cause the interacting. For example, when $Z$ is high, the interacting probability will be increased, because the there are some social effect exist, such as user interest will be influenced by the majority of groups, and the interest will be increased with high item popularity, such as the interest for news that becomes hot. In the graph, we can find there are two paths from $Z$ to $C$, one is the above $Z \rightarrowI C$, the another is $Z \rightarrow I \ right C $. The latter one is that what we don't need. We need cut off $Z \rightarrow I $ to prevent the confounding effect caused by it. % 感觉应该说 I <- Z -> C，Z-> I -> C 不是很明白。


% Figure~\ref{fig:rec_graph}(b) shows the causal graph that abstracts the generation process of historical data where the variable $Z$ affects both $I$ and $C$, \ie $Z$ is a \textit{confounder} between $I$ and $C$~\cite{pearl2009causality}. 
% Due to the existence of $Z$, estimating $P(C | U,I)$ from the historical data will suffer from spurious correlation~\cite{pearl2009causality}, leading to popularity bias amplification, \ie popular items are over-recommended. Note that most existing recommender systems estimates the correlation $P(C|U, I)$ by optimizing a recommendation loss over the historical data.
% such as the BPR Loss~\cite{bpr} over the historical data, which is formulated as:
% \begin{equation}\label{eq:bpr}
%     \min \sum_{(u, i^{+}/i^{-}, c) \in \mathcal{D}/\mathcal{D}^-} -log( \sigma(P(c |u, i^{+}) - P(c |u, i^{-})) ),
% \end{equation}
% where $\mathcal{D}^-$ denotes randomly selected negative samples and $\sigma(\cdot)$ is the sigmoid activation function. 
% Obviously, the correlation can be separated into two parts:
% \begin{equation} \label{eq:bayes-pop-bias}
%   P(C|U,I) = \sum_z P(C|U,I,z)P(z|I).
% \end{equation}
% %%%
% % TODO: check if it is correct
% %%%
% $P(C|U,I)$ will be easily dominated by the $P(C|U,I,z)$ with higher $P(z|I)$ (note that $U$ is independent to $Z$ in the graph). Between two items, the popular one has larger $P(z|I)$ since the popular item is typically recommended more frequently, for the $z$ that usually has higher $P(C|U,I,z)$. %and the $P(C|U,I,z)$ corresponding to these $z$ usually has higher values than others.
% Therefore, the correlation of the popular item will be amplified, which thus calls for the consideration of cutting off $Z \rightarrow I$ during recommender model training.

%%%
% TODO: use the version without M
%%%
% \begin{table}[h]
% %\caption{An example for our graph}
% \caption{An example to show popularity bias amplification.}
% \vspace{-0.3cm}
% \label{tab:example_confounder}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% $C$ & $I$ & $Z$ & $P(Z|I)$ & $P(C|u,I,Z)$ & 
% % \begin{minipage}{1in}
% % \begin{equation*}
% %     \begin{split}
% %       &P(C|u,I) = \\
% %       & \sum P(C|u,I,z_j)P(z_j |I)  
% %     \end{split}
% % \end{equation*}
% % \end{minipage}
% $ P(C|u,I) $ %sum P(C|u,I,z_j)P(z_j |I)
% \\ \hline
% \multirow{4}{*}{1} & \multirow{2}{*}{$i_1$} & $z_1$ & 0.60 & 0.75 & \multirow{2}{*}{0.65} \\ \cline{3-5}
%  &  & $z_2$ & 0.40 & 0.50 &  \\ \cline{2-6} 
%  & \multirow{2}{*}{$i2$} & $z_1$ & 0.40 & 0.75 & \multirow{2}{*}{0.60} \\ \cline{3-5}
%  &  & $z_2$ & 0.60 & 0.50 &  \\ \hline
% \end{tabular}
% \end{table}

% \paragraph{Example.} We then perform a quantitative analysis with a simple instantiation of the generation process, where $\mathcal{U} = \{u\}$, $\mathcal{I} = \{i_1, i_2\}$, and $\mathcal{Z}=\{z_1, z_2\}$. 
% We assume that: (1) $i_1$ is more popular than $i_2$; (2) $z_1$ and $z_2$ are two potential recommendation strategies with equal probabilities, \ie $P(z_1) = P(z_2)$; (3) the popularity bias affects $z_1$ more than $z_2$, \ie $P(i_1 | z_1) = 0.6$ but $P(i_1 | z_1) = 0.4$, which means $z_1$ recommends more popular items; and (4) the user has equal interest to the two items, which means that $P(C|u,i_1,Z) = P(C|u,i_2,Z)$, \ie $I=i_1$ and $I=i_2$ have the same effect on $C$. 
% Table~\ref{tab:example_confounder} shows the detail of estimating $P(C|u,I)$. From the table, we can see that $P(C|u,i_1)$ is great than $P(C|u,i_2)$, which is indeed popularity bias amplification. Ideally, the two items should receive the same recommendation score.
% Through simple calculation, we find that the correlation $P(C|u,I)$ is dominated by $P(C|u,I,z_1)$ where $P(z_1 | i_1 )$ is great than $P(z_1  | i_2 )$. It reveals the reason of popularity bias amplification, \ie the effect from $Z$ to $I$.


% From the result, we can find that $P(z_1  | i_1 )$ is great than $P(z_1  | i_1 )$, and the corresponding $P(z | u,I , z_1 )$ has the higher than $P(z | u,I , z_2 )$
% Assuming that the user has equal interest to the two items with probability $p=0.5$ to click both $i_1$ and $i_2$, \ie the estimated interests should be equal for the two items. And assume that $\mathcal{Z}=\{z_1, z_2 \}$ withe same probability for the $z_1$ and $z_2$. And $Z=z_1$ ($z_2$), $i_1$ will appear with $p=0.6 (0.4)$, and $i_2$ will appear with $p=0.4 (0.6)$. What more when the $Z=z_1 $, the click probability will increase $1/4$ whatever $I$ is, \ie $P(C|u,I,z_1) = 0.75$, and assume $z_2$ has not influence on $C$. Then we can compute $P(C|u,i)$ as Table~\ref{tab:example_confounder}. From the result, we can find that $P(z_1  | i_1 )$ is great than $P(z_1  | i_1 )$, and the corresponding $P(z | u,I , z_1 )$ has the higher than $P(z | u,I , z_2 )$, lead to $P(C|u,i_1)$ is great than $P(C|u,i_2 )$. While the true interests for two items are equal.   

% Furthermore, we give a simple example based on our causal graph for recommendation: Let $\mathcal{U} = \{u_1\}$, and $Z$ has two types of values $1,-1$ with different probabilities $[0.6,0.4]$. And there are two items $i_1 ,i_2 $ and one user $u_1$ which has basic  $1/2$ probability to click the item. $I$ has 0.6 (0.4) probability to take $i_1 $, and 0.4 (0.6) probability to take $i_2$ when $Z=1 (-1)$. 
% %To simply, let $f_M(Z,I)=Z$ to represent current popularity, and "-1" represent popular. 
% And if $M=1$ (popular) the click rate for the item will increase 1/4, else decrease 1/4, the strucal functions can be summarised as:  

% \paragraph{Simulation experiment.} To further demonstrate the analysis, we conduct a simulation experiment with a simple instantiation of the generation process, where $\mathcal{U} = \{u_1\}$ and $\mathcal{I} = \{i_1, i_2\}$. Assuming that the user has equal interest to the two items, \ie 
% Furthermore, we give a simple example based on our causal graph for recommendation: Let $\mathcal{U} = \{u_1\}$, and $Z$ has two types of values $1,-1$ with different probabilities $[0.6,0.4]$. And there are two items $i_1 ,i_2 $ and one user $u_1$ which has basic  $1/2$ probability to click the item. $I$ has 0.6 (0.4) probability to take $i_1 $, and 0.4 (0.6) probability to take $i_2$ when $Z=1 (-1)$. 
% %To simply, let $f_M(Z,I)=Z$ to represent current popularity, and "-1" represent popular. 
% And if $M=1$ (popular) the click rate for the item will increase 1/4, else decrease 1/4, the strucal functions can be summarised as:  
% \begin{equation}
%     \begin{split} 
%         &\mathcal{U} = \{u_1\}, \mathcal{I} = \{i_1,i_2\}, Z=\{z_1, z_2 \}\\
%         &f_Z = \text{ with p=0.6 and -1 with 0.4}\\
%         & f_I = \begin{cases}
% 	\text{$i_1$ with p =0.6 and $i_2$ with p=0.4}, &\text{if } Z=1 \\
% 	\text{$i_1$ with p =0.4 and $i_2$ with p=0.6}, &\text{if } Z=-1
% 		   \end{cases} \\
% 		   % &f_X = if\,Z=-1 (1) \, i_1 \, P= 0.6 (0.4); i_2 \, p=0.4 (0.6) \\
%         % &f_M = Z \\
%         &f_C =  1 \,with \, p = 0.5 + 0.25 sgn(Z) \text{\, for both $i_1$ and $i_2$}
%     \end{split}
% \end{equation}
% Where $p$ refers to probability corresponding to one event, and $sgn(\cdot)$ is sign function.



% \begin{table}[]
% \caption{The generated data by the assumed model based our recommendation graph. The values such as 36(27) represents 36 times recommendation and 27 times clicking.}
% \label{tab:example}
% \begin{tabular}{lll}
% \hline
% \multicolumn{1}{l|}{Z\textbackslash{}I} & $i_1$ & $i_2$ \\ \hline
% \multicolumn{1}{l|}{1} & 36(27) & 24(18) \\ \hline
% \multicolumn{1}{l|}{-1} & 16(4) & 24(6) 
% \end{tabular}
% \end{table}
% And we generate data by simulating the above mechanism 100 times, we can get data like \ref{tab:example}.  The real interests for the two items should be $0.5$ according to $f_C$. But it's easy to compute that $P(C=1|i_1, u_1) = 0.596\, P(C=1|i_2, u_1) = 0.5 $. It obviously that the interest for $i_1$ has been amplified.  This is an example of spurious correlation that will influce the estimate user's real interests. This is the confounding effect.

\subsection{Deconfounded Training}\label{ssec:PD}
We now consider how to obtain a model that is immune to the impact of $Z\rightarrow I$. Intuitively, if we can intervene the exposure mechanism to make it randomly expose items to users, then the collected interaction data is free from the impact of $Z\rightarrow I$. Directly training traditional models on it will do. However, the feasibility and efficacy of such solutions are low: first, only the recommender builder can intervene the exposure mechanism, and anyone else (\eg academia researcher) has no permission to do it; second, even for recommender builder that can intervene the exposure mechanism, they can only use small random traffic, since random exposure hurts user experience much. Effective usage of small uniform data remains an open problem in recommendation research~\cite{2018causalE, distillation}. 

Fortunately, the progress of causal science provides us a tool to achieve intervention without performing the interventional experiments~\cite{pearl2009causality}. The secret is the \textit{do}-calculus. In our context, performing $do(I)$ forces to remove the impact of $I$'s parent nodes, achieving our target. As such, we formulate the predictive model as $P(C| do(U, I) )$, rather than $P(C| U, I )$ estimated by traditional methods\footnote{Note that since there is no backdoor path between $U$ and $C$ in our causal graph, it holds that $P(C| U, do(I) ) = P(C| do(U), do(I) ) = P( C| do (U, I))$. Here we use $P(C| do(U, I) )$ as the intervention model for brevity. }. %\footnote{Note that since $U$ has no parents in our causal graph, it holds that $P(C| U, do(I) ) = P(C| do(U), do(I) ) = P( C| do (U, I))$. Here we use $P(C| do(U, I) )$ as the intervention model for brevity. }. 

Let the causal graph shown in Figure~\ref{fig:rec_graph}(b) be $G$, and the intervened causal graph shown in Figure~\ref{fig:rec_graph}(c) be $G'$. Then, performing \textit{do}-calculus on $G$ leads to:
\begin{equation}\label{eq:do-derivation}\small
	\begin{split}
	P(C|do(U,I)) & \overset{(1)}{=}  P_{G'} (C|U,I)\\
	& \overset{(2)}{=} \sum_z P_{G'}(C|U,I,z)P_{G'}(z|U,I)\\
	& \overset{(3)}{=} \sum_z P_{G'}(C|U,I,z)P_{G'}(z)\\
	& \overset{(4)}{=} \sum_z P(C|U,I,z) P(z),
	\end{split}
\end{equation}
where $P_{G'}(\cdot)$ denotes the probability function evaluated on $G'$. Below explains this derivation step by step: 
\begin{itemize}[leftmargin=*]
    \item (1) is because of \textit{backdoor criterion}~\cite{pearl2009causality} as the only backdoor path $I\leftarrow Z \rightarrow C$ in $G$ has been blocked by $do(U, I)$;
    \item (2) is because of Bayes' theorem;
    \item (3) is because that $U$ and $I$ are independent with $Z$ in $G'$; 
    \item (4) $P(C|U,I,Z) = P_{G'}(C|U,I,Z)$ is because that the causal mechanism $\{U,I,Z\}\rightarrow C$ is not changed when cutting off $Z\rightarrow I$, $P(Z) = P_{G'}(Z)$ since $Z$ has the same prior on the two graphs.
\end{itemize}

Next, we consider how to estimate $P(C|do(U, I))$ from data. Apparently, we need to first estimate $P(C|U,I,Z)$, and then estimate $\sum_z P(C|U,I,z) P(z)$. \vspace{+5pt}

\noindent \textbf{Step 1. Estimating $P(C|U,I,Z)$.} This conditional probability function evaluates that given a user-item pair $U=u, I=i$ and the item's present popularity as $Z=m_i^t$, how likely the user will consume the item. Let the parameters of the conditional probability function be $\Theta$, we can follow traditional recommendation training to learn $\Theta$, for example, optimizing the pairwise BPR objective function on historical data $\mathcal{D}$: 
\begin{equation}\label{eq:bpr}\small
    \max_{\Theta} \sum_{(u, i, j) \in \mathcal{D}} \text{log} \sigma \left(
        P_\Theta\left(
            c=1 | u, i, m_{i}^{t}
        \right) - P_\Theta \left(
            c=1 | u, j, m_{j}^{t}
        \right) 
    \right),
\end{equation} 
where $j$ denotes the negative sample for $u$, $\sigma(\cdot)$ is the sigmoid function. The $L_2$ regularization is used but not shown for brevity.  

Having established the learning framework, we next consider how to parameterize $P_\Theta(c=1 | u, i, m_{i}^{t})$. Of course, one can design it as any differentiable model, factorization machines, or neural networks. But here our major consideration is to decouple the user-item matching with item popularity. The benefits are twofold: 1) decoupling makes our framework extendable to any collaborative filtering model that concerns user-item matching; and 2) decoupling enables fast adjusting of popularity bias in the inference stage (see Section~\ref{sec:PDA}), since we do not need to re-evaluate the whole model. To this end, we design it as:
\begin{equation} \label{eq:model}\small
    P_\Theta(c=1 | u, i, m_{i}^{t}) = ELU'(f_\Theta(u, i)) \times ({m}_{i}^{t})^\gamma,
\end{equation}
where $f_\Theta(u, i)$ denotes any user-item matching model and we choose the simple \textit{Matrix Factorization} (MF) in this work; hyper-parameter $\gamma$ is to smooth the item popularity and can control the strength of conformity effect: setting $\gamma=0$ means no impact and larger value assigns larger impact. $ELU'(\cdot)$ is a variant of the Exponential Linear Unit \cite{elu} activation function that ensures the positivity of the matching score:
\begin{equation} \label{eq:alph-example}\small
	ELU'(x) = \begin{cases}
	e^{x}, &\text{if } x \leq 0 \\ 
	x+1, &\text{else}  %\in \mathbb{R}\setminus\mathbb{Q}	
		   \end{cases}
\end{equation}
This is to ensure the monotonicity of the probability function since $({m}_{i}^{t})^\gamma$ is always a positive number. Lastly, note that one needs to normalize $ P_\Theta(c=1 | u, i, m_{i}^{t})$ to make it a rigorous probability function, but we omit it since it is time-consuming and does not affect the ranking of items. \vspace{+5pt}

% \begin{algorithm}[t]
% 	\caption{Popularity-bias Deconfounding(PD)}
% 	\LinesNumbered
% 	\label{alg:PD-learing}
% 	\KwIn{Dataset $\mathcal{D}=\{D_1,\dots,D_{T}\}$}
% % 	\KwOut{Updated recommender $W_{t+1}$}
% % 	Split D to T chunks \{$D_1,\dots,D_{T-1}$\} along time \;
%     // Step 1: estimate $P(C|U,I,Z)$ \;
% 	Compute each item $i$ popularity $m_{i}^{t}$ on each stage $t$ by Equation \eqref{eq:pop_define} \;
% 	Match each interaction $(u,i)$ in stage $t$ with $m_{i}^{t}$\;
% 	\While{Stop condition is not reached}{
% 	Randomly sample one batch interactions $B$ in $\mathcal{D}$\;
% 	Compute $f(u,i,m_{i}^{t})$\;
% 	Update model parameters by optimizing Equation~\ref{eq:loss}. 
% 	}
% 	// Step 2: inference with $P(C|do(U,I))$ \;
% 	Ranking items with $\alpha(k_{u,i})$
	
% \end{algorithm}

\noindent \textbf{Step 2. Estimating  $\sum_z P(C|U,I,z) P(z)$.} Now we move forward to estimate the interventional probability $P(C|do(U, I))$. Since the space of $Z$ is large, it is inappropriate to sum over its space for each prediction evaluation. Fortunately,  we can perform the following reduction to get rid of the sum:
%With the estimation of $P(C|U,I,Z)$, we can approximate this intervention probability as:
\begin{equation}\label{eq:doUI}\small
   \begin{split}
    P(C|do(U,I)) &= \sum_{z} P(C|U,I,z)P(z) \notag\\
    & = \sum_z ELU'(f_{\Theta}(u,i)) \times z^{\gamma} P(z) \\
    & = ELU'(f_{\Theta}(u,i)) \sum_z z^{\gamma}P(z) \\
    & = ELU'(f_{\Theta}(u,i)) E(Z^{\gamma})
\end{split} 
\end{equation}
where $E(Z^{\gamma})$ denotes the expectation of $Z^{\gamma}$. Note that the expectation of one variable is a constant. Since $P(C|do(U, I))$ is used to rank items for a user, the existence of $E(Z^{\gamma})$ does not change the ranking. We can thus use $ELU'(f_{\Theta}(u,i))$ to estimate $P(C|do(U, I)$. \vspace{+5pt}

%the goal of recommendation is to rank items for a user. Ranking with $P(C|do(U,I))$ is equal to ranking with $ELU(f_{\Theta}(u,i))$.

\noindent To summarize, we fit the historical interaction data with $P_\Theta(c=1|u, i, m_i^t)$, and use the user-item matching component $ELU'(f_{\Theta}(u,i))$ for deconfounded ranking. We name this method as \textit{Popularity-bias Deconfounding} (PD).


% Considering that we are unable to enumerate the instance of $Z$, we first derive an approximation of $P(C|do(U,I))$. Formally,
% \begin{align}
%     P(C|do(U,I)) &= \sum_z P(C|U,I,z)P(z) \notag\\
%     & \approx P(C|U,I,E(Z)),
% \end{align}
% where $E(Z)$ denotes the expectation of $Z$. It should be noted that $E(Z)$ is constant and not depends on the value of $I$. We can thus approximate $P(C|U,I,E(Z))$ by setting the $m_i^t$ in $h(u,i,m_i^t)$ with a proper constant value, \ie $h(u,i,m^*)$. As the value of $m^*$ does not change the ranking of items, we simply set $m^* = 1$. That is to say, we estimate $P(C|do(U,I))$ as $\alpha(k_{ui})$.



%%%
% TODO: fill in the contents and rephrase
%%%
% In Algorithm \ref{alg:PD-learing}, we summarize the process of PD, which has two main differences to the existing methods:
% \begin{itemize}[leftmargin=*]
%     \item PD estimates $P(C|U,I,Z)$ during recommender training instead of $P(C|U,I)$.
%     \item PD makes recommendation with $P(C|do(U,I))$ instead of $P(C|U,I)$.
% \end{itemize}

%At last, we summarize the process of our PD in Algorithm \ref{alg:PD-learing}.
%  \subsection{Inference with drifted popularity}

%%%
% TODO: update the contents to be coherent with the previous subsection
%%%
\subsection{Adjusting Popularity Bias in Inference}\label{sec:PDA}
Owing to $P(C|do(U, I))$, we can eliminate the bad effect of popularity bias. We now seek for better usage of popularity bias, \eg promoting the items that have the potential to be popular. 
Assume the target popularity bias is $\Tilde{z}$, and we want to endow the recommendation policy with this bias. To achieve the target, we just need to do the intervention of $Z=\Tilde{z}$ for model inference:
\begin{align}\small\label{eq:do-z}
    P(C|do(U=u,I=i),do(Z=\Tilde{z})) = P_\Theta(c=1|u,i, \Tilde{m}_i),
\end{align}
where $\Tilde{m}_i$ denotes the popularity value of $\Tilde{z}$. 
This intervention probability directly equals the conditional probability since there is no backdoor path between $Z$ and $C$ in the causal graph. %$Z$ has no parents in the causal graph.
%Since the derivation step is similar to the Equation~\eqref{eq:do-derivation}, we omit it here. According to the formulation of Step 1, we can approximate it with $P_{\Theta}(C|u,i, \Tilde{z})$. Assume the desired popularity for item $i$ is $\Tilde{m_i}$,  $P_{\Theta}(u,i,\Tilde{m}_i)$ is used for inference. 
% Considering the need of introducing desired popularity bias into the system, such as promoting the items that have the potential to be popular, the core is equal to adjust the popularity be the same to the desired one by force. To realize this goal, we can intervene $Z=\Tilde{z}$ that corresponds to the desired item popularity, and can intervene $U=u$ and $I=i$ to simulate the responses,\ie $P(C|do(U=u,I=i),do(Z=\Tilde{z}))$. Then we can recommend item with the responses to do real recommendation to get higher recommendation accuracy. For  $P(C|do(U=u,I=i),do(Z=\Tilde{z}) )$, according to back-door adjustment, we have:  %we only need to cut down the paths that arrow into $Z$ of the right graph in figure~\ref{fig:rec_causal_pre_now}.There are not any these types of paths. So we can compute it still on the right graph, we can get:
%  \begin{equation}
%  P(C|do(U=u,I=i),do(Z= \Tilde{z} )) = P(C|u,i,\Tilde{z} ) 
%  \end{equation}
Since the focus of this work is not on popularity prediction, we employ a simple time series forecasting method to set $\Tilde{m}_i$: 
\begin{equation}\small \label{eq:pre_pop}
    \Tilde{m}_i = m_{i}^{T} + \alpha (m_{i}^{T} - m_{i}^{T-1}),
\end{equation}
where $m_{i}^{T}$ is the popularity value of the last stage, and $\alpha$ is the hyper-parameter to control the strength of popularity drift in predicting the future. We name this method as \textit{Popularity-bias Deconfounding and Adjusting} (PDA). 

%Both Figure \ref{fig:framework} and Algorithm \ref{alg:PD-PDA} summarize our method. The training stage optimizes Equation~(\ref{eq:bpr}) (line 2 in the algorithm). The inference stage can adjust the popularity bias (line 7 in the algorithm) as:
Figure \ref{fig:framework} illustrates the workflow of PDA where the training stage optimizes Equation~(\ref{eq:bpr}) and the inference stage can adjust the popularity bias as:
% \begin{equation}\label{eq:mf}\small
%      PDA_{ui} = ELU'(f_\Theta(u, i)) \times (\Tilde{m}_i)^{\Tilde{\gamma}}.
% \end{equation}
\begin{equation}\label{eq:mf}\small
     PDA_{ui} = ELU'(f_\Theta(u, i)) \times (\Tilde{m}_i)^{\Tilde{\gamma}}.
\end{equation}
$\Tilde{\gamma}$ denotes the popularity smoothing hyper-parameter used for model inference, which can be different from that used in training.
This is to consider that the strength of popularity bias can drift in the future. 
In practice, setting $\Tilde{\gamma} = \gamma$ can achieve expected performance (\cf Table~\ref{tab:PDA-result}). 
Setting $\Tilde{\gamma}=0$  degrades the method to PD that uses only interest matching for recommendation. Considering the importance of properly stopping model training, PDA uses a model selection strategy based on the adjusted recommendation, which is slightly different from that of PD (see Algorithm \ref{alg:PD-PDA}).
% Ideally, if we have the ground truth of $P(C|do(U,I))$ to select a best model, we think that the model parameters $\Theta$ trained for PD can be used for PDA directly. But there is not the ground-truth. In practice, we will tune the hyper-parameter $\gamma$ in training again and select a more appropriate $\Theta$ for PDA (line 4 of the algorithm). Meanwhile, for simplicity, we keep $\Tilde{\gamma}$ as the newfound one.


%Note that we do not use more complicated time-series forecasting methods such as Recurrent Neural Network~\cite{}, since we find that the simple algorithm is sufficient to achieve good results (\cf Table/Figure XX).
%%%
% TODO: need to explain why don't use more complex models.
%%%
%%%
% TODO: view (a) as an ablation study without the forecast
%%%
%We take two methods to predict the desired popularity for $\mathcal{D}_{T+1}$: (a) the first is that treat the item popularity in $D_{t}$ as the predicted popularity, With the fact that the item popularity in the most near stage has the small popularity drift as showing in~\ref{fig:drit_showing}. (b) the second is $\Tilde{m}_i = m_{i}^{T} + \alpha (m_{i}^{T} - m_{i}^{T}) $, in this form, besides considering the most recent item popularity as a import information, taking the item popularity difference on the most recent two stage term as drifting trends.   

%%%
% TODO: add framework figure here
%%%
\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{figures/framework_5.pdf} %framwork-nosampling
    \vspace{-0.4cm}
    \caption{The workflow of our method. The blue arrows represent the training stage and the red arrows represent the inference stage.}
    \label{fig:framework}
    \vspace{-13pt}
\end{figure}

% \paragraph{Instantiation on Matrix Factorization.}
% To demonstrate how our proposed PDA framework works, we provide an implementation based on \textit{Matrix Factorization} (MF), which is a representative embedding model for recommendation. Given a user-item pair
% $(u,i)$, the user-item matching given by PD and PDA are:

% \begin{equation}\label{eq:mf}
%      PD_{ui} = ELU(p_{u}^{\top} q^{i}),~PDA_{ui} = ELU(p_{u}^{\top} q^{i}) \times (\Tilde{m}_i)^{\gamma},
% \end{equation}

% \begin{equation}\label{eq:mf}
%      PD_{ui} = \alpha(p_{u}^{\top} q^{i}),~PDA_{ui} = \alpha(p_{u}^{\top} q^{i}) \times (\Tilde{m}_i)^{\gamma},
% \end{equation}
 
%  MF predicts the user-item matching as
%  \begin{equation}\label{eq:mf}
%      k_{ui} = p_{u}^{\top} q^{i}
%  \end{equation}

% where $p_{u} \in \mathbb{R}^d$ and $p_{u} \in \mathbb{R}^{d}$ represent the the embedding of $U=u$ and $I=i$ respectively, and $d$ is the embedding size. 

%We take the $\alpha(\cdot)$ for equation \eqref{eq:alph-example} and $\beta_{1}$ as the activation functions  for \eqref{eq:do-re-scale}.
%  $$ f(u,i,m_{i}^{t} ) = \alpha(k_{ui})\times (\hat{m}_{i}^{t})^{\gamma} $$.
% For recommendation Loss $L_0$, 
% We adopt BPR loss in equation~\ref{eq:loss}, which is a common choice for recommendation models. And for each positive samples, we randomly sample 1 unobserved interaction for each positve one.
% For each $(u,i,m_{i}^{t})$, we randomly sample 1 unobserved interaction of u, denoting its item as $i^{-}$, to represent negative interaction. We take $m_{i^{-}}^{t}$ as the item popularity for the interaction. 

%Then BPR loss is formulated as:
% \begin{equation}
%     L_{0} (P,Q|D) = \sum_{(u,i,i^{-},t,m_{i}^{t})\in D} log(\sigma(f(u,i,m_{i}^{t} ) - f(u,i^{-}, m_{i^{-}}^{t}))) 
% \end{equation}
% where $P,Q$ denote the embeddings of all users and items, and $\sigma(\cdot)$ is the sigmoid function.

%%%
% TODO: only keep two main points: 1) contents from explaining the causal graph (without the example) to why NDE; 2) derivative and explain why \alpha(k_{ui}) is equivalent to NDE.

\subsection{Comparison with Correlation $P(C|U, I)$}
In the beginning, we argue that traditional methods estimate the correlation $P(C|U, I)$ and suffer from the bad effect of popularity bias amplification. Here we analyze the difference between $P(C|U, I)$ and $P(C|do(U, I))$ to offer more insights on this point.

We first transform $P(C|U, I)$ with the following steps:
\begin{equation}\small
    \begin{split}
        P(C|U,I) & \overset{(1)}{=} \sum_{z} P(C,z|U,I) \\
        & \overset{(2)}{=} \sum_{z} P(C|U,I,z)P(z|U,I) \\ 
        & \overset{(3)}{=} \sum_{z} P(C|U,I,z)P(z|I) \\
        & \overset{(4)}{\propto	} \sum_{z} P(C|U,I,z)P(I|z)P(z)  
    \end{split}
\end{equation}
(1) is the definition of marginal distribution; (2) is because of the Bayes' theorem; (3) is because $U$ is independent to $Z$ according to the causal graph; (4) is because of the Bayes' theorem. 

Comparing with $P(C|do(U,I)) = \sum_{z} P(C|U,I,z) P(z)$,
% \begin{equation}\nonumber \small
%   P(C|do(U,I)) = \sum_{z} P(C|U,I,z) P(z). 
% \end{equation}
% $$P(C|do(U,I)) = \sum_{Z} P(C|U,I,Z) P(Z). $$ 
we can see that $P(C|U, I)$ has an additional term: $P(I|Z)$, which fundamentally changes the recommendation scoring. Suppose $I=i$ is a popular item, $P(C|U, I=i, Z=m_i^t)$ is a large value since $m_i^t$ is large, which means the term has a large contribution to the prediction score. $P(I=i | Z=m_i^t)$ is also a large value due to the popularity bias in the exposure mechanism. Multiplying the two terms further enlarges the score of $i$, which gives $i$ a higher score than it deserves. As a result, the popularity bias is improperly amplified. This comparison further justifies the rationality and necessity of $P(C|do(U,I))$ for learning user interests reliably.  

%Compare $P(C|U,I)$ with $P(C|do(U,I))$,
%$$P(C|U,I) = \sum_{z} P(C|U,I,z) P(z|I) $$
%$$P(C|do(U,I)) = \sum_{z} P(C|U,I,z) P(z) $$
%They differ in the second term. We can treat them as sum $P(C|U,I,Z)$ over $Z$ with different wights for different $Z$. For $P(C|do(U,I))$, the weights is $P(Z)$, for $P(C|U,I)$ is the $P(Z|I)$. 

%Assume that $P(C|U,I,z)$ contains two parts of effects --- interest effect and the direct effect from $Z\rightarrow C$, and for a fixed $z$, direct effect from $Z \rightarrow I$ will not changed for $I$. Note that in $P(C|do(U,I))$, each $P(C|U,I,z)$ will has the same weight $P(z)$ whatever the $I$ is. So the summed direct effects from $Z\rightarrow C$ in $P(C|do(U,I))$ will be same for different $I$. So we compare $P(C|do(U,I))$ is equal to compare interest.

%While for $P(C|U,I)$, some items will pay more weights to $P(C|U,I,z)$ with high $z$, while other items will pay more attention to $P(C|U,I,z)$ with low $z$. Meanwhile, $P(C|U,I,z)$ with high $z$ contains high direct effects from $Z \rightarrow C$. That means $P(C|U,I)$ for these items has higher summed direct effects from $Z \rightarrow C$. While the $P(C|U,I)$ for the other items has lower summed direct effects from $Z \rightarrow C$. So comparing $P(C|U,I)$ between different $I$ will be influenced by the different level of summed direct effects from $Z \rightarrow C$. So weights allocation policy decisions result in mislead.   

%Indeed, we can think it simulates a intervention experiment: making each $I$ has the same probability to popular by force, and also has the same probability to unpopular by force, and assume the direct effect of $Z$ to $C$ will not influenced by $I$. 

% Because each $I$ has the same probability to whatever a $Z$, the effect of $Z$ to $C$ will be same for all items, that is we are compare the effect caused by different $I$. But for $$P(C|U,I)$$, the weights will be difference for different items. Some items have high weight on $Z$ represent high popularity, and for this $Z$ it will has high effect on $C$, that is the effect of $Z$ to $C$ will be different for different $I$.        
%it will not influenced by which $I$ is. It simulate a intervention experiment that:        

%%%%%%%%%%%% previous version.
% Obviously, the correlation can be separated into two parts:
% \begin{equation} \label{eq:bayes-pop-bias}
%   P(C|U,I) = \sum_z P(C|U,I,z)P(z|I).
% \end{equation}
% Comparing it with
% $$ P(C|do(U,I)) = \sum_z P(C|U,I,z)P(z), $$
% the difference is that $P(C|do(U,I))$ take $p(z)$ while the correlation take $(C|U,I,z)$ to weighting $P(C|U,I,z)$ in the equation. $p(z)$ is mean to that the value of $z$ is not influenced by $I$, then we can think $do(U,I)$ is to answer the question what the result will be, if place $I$ to different $Z$ with same probability $P(z)$ for different items. In this way the path between $I$ and $Z$ has been cut off. But for $P(C|U,I)$, it takes $P(z|I)$, that means for a same $z$, some items has higher probability while others with low probabilty. For a popular item, $P(C|u,i,z)p(z|i) $ pay more attention to the term $P(C|u,i,z)$ with high z, which is usually the term with high value. While the unpopular item will more concentrate on the term $P(C|u,i,z)$ with low $z$ which usually means the term with low values, because of $P(z|i)$ is high for the low $z$. Relatively speaking, $P(C|u,i)$ for popular items will be amplified than the unpopualr items.

%%%
% TODO: check if it is correct
%%%
% $P(C|U,I)$ will be easily dominated by the $P(C|U,I,z)$ with higher $P(z|I)$ (note that $U$ is independent to $Z$ in the graph). Between two items, the popular one has larger $P(z|I)$ since the popular item is typically recommended more frequently, for the $z$ that usually has higher $P(C|U,I,z)$. %and the $P(C|U,I,z)$ corresponding to these $z$ usually has higher values than others.
% Therefore, the correlation of the popular item will be amplified, which thus calls for the consideration of cutting off $Z \rightarrow I$ during recommender model training.

%%%
% TODO: use the version without M
%%%



% \begin{table}[h]
% %\caption{An example for our graph}
% \caption{An example to show popularity bias amplification.}
% \vspace{-0.3cm}
% \label{tab:example_confounder}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% $C$ & $I$ & $Z$ & $P(Z|I)$ & $P(C|u,I,Z)$ & 
% % \begin{minipage}{1in}
% % \begin{equation*}
% %     \begin{split}
% %       &P(C|u,I) = \\
% %       & \sum P(C|u,I,z_j)P(z_j |I)  
% %     \end{split}
% % \end{equation*}
% % \end{minipage}
% $ P(C|u,I) $ %sum P(C|u,I,z_j)P(z_j |I)
% \\ \hline
% \multirow{4}{*}{1} & \multirow{2}{*}{$i_1(pop)$} & $z_1(pop)$ & 0.60 & 0.75 & \multirow{2}{*}{0.65} \\ \cline{3-5}
%  &  & $z_2(unpop)$ & 0.40 & 0.50 &  \\ \cline{2-6} 
%  & \multirow{2}{*}{$i_2$} & $z_1$ & 0.40 & 0.75 & \multirow{2}{*}{0.60} \\ \cline{3-5}
%  &  & $z_2(unpop)$ & 0.60 & 0.50 &  \\ \hline
% \end{tabular}
% \end{table}

% \paragraph{Example.} To show problem of $P(C|U,I)$. We perform a quantitative analysis with a simple instantiation of the generation process, where $\mathcal{U} = \{u\}$, $\mathcal{I} = \{i_1, i_2\}$, and $\mathcal{Z}=\{z_1(pop), z_2(unpop)\}$. We assume that: (1) $i_1$ is more popular than $i_2$; (2) $z_1$ and $z_2$ are two potential recommendation strategies with equal probabilities, \ie $P(z_1) = P(z_2)$; (3) the popularity bias affects $z_1$ more than $z_2$, \ie $P(i_1 | z_1) = 0.6$ but $P(i_1 | z_1) = 0.4$, which means $z_1$ recommends more popular items; and (4) the user has equal interest to the two items, which means that $P(C|u,i_1,Z) = P(C|u,i_2,Z)$, \ie $I=i_1$ and $I=i_2$ have the same effect on $C$.Table~\ref{tab:example_confounder} shows the detail of estimating $P(C|u,I)$. From the table, we can see that $P(C|u,i_1)$ is great than $P(C|u,i_2)$, which is indeed popularity bias amplification. Ideally, the two items should receive the same recommendation score.Through simple calculation, we find that the correlation $P(C|u,I)$ is dominated by $P(C|u,I,z_1)$ where $P(z_1 | i_1 )$ is great than $P(z_1  | i_2 )$. It reveals the reason of popularity bias amplification, \ie the effect from $Z$ to $I$.




% To estimate true interest we must remove the confounding effect. The idea way is to do intervention experiment, but it's not practical for our works. To remove the confounding effect from observed data. The key is to control (condition on) the confounder or the variable that is descendant of confounder instead of the cause($I$ in here). $Z$ can satisfy this condition, but unfortunately, Z is not observable. We can only to control $M$, a  descendant of both $Z$ and $I$. The influence of controlling $M$ will cut down the causal path $I\rightarrow M \rightarrow C$, but fortunately, even though the path also will cause $C$, it is not what we need because is caused through conformity instead of interest. What's more, $M$ can computed from data. With this idea, we can estimate $P(C|U,I,M)$ from data, and comparing user interest for different items by Natural Direct Effect (NDE), which compares the causal effect condition on the same whatever $M$. According to \cite{hanwang_longtail}, NDE can be approximated as following: 
% \begin{equation} \label{eq:nde}
% \begin{split}
%     NDE(C=1|u,i) & = P(C|do(u,i),M=m^* ) - P(C|do(u,i^* ),m=m^* ) \\
%     &= P(C|u,i,m^* ) - P(C|u,i^* ,m^* )
% \end{split}
% \end{equation}
% , where $do$ means intervene on the variable, and $i^*$ and $m^*$ is dummy value. And because we do ranking tasks, we can directly to compare $P(C|u,i,m^* )$ between items for the user $u$. Estimating the $P(C|U,I,M)$ with the same form in equation~\eqref{eq:do-matching}, ranking will still be the same term $\alpha(K_{ui})$.

%Return to the real-world recommendations, previous work CF methods directly model $P(C|U,I)$ to fit data, it obviously will be influenced by the confounding. To solve the problem, we must to remove the confounding effect. The idea way is to do intervention experiment, but it's not practical for our works. To remove the confounding effect from observed data, back-door-adjustment introduced in~\cite{pearl_primer,pearl2009causality} can be used. The key is to control (condition on) the confounder or the variable that is descendant of confounder instead of the cause, $I$ in here. Z can satisfy this condition, but unfortunately, Z is not observable. We can only to control $M$, a  descendant of both $Z$ and $I$. The influence of controlling $M$ will cut down the causal path $I\rightarrow M \rightarrow C$, but fortunately, even though the path also will cause $C$, it is not what we need because is caused through conformity instead of interest. And what's more$M$ can computed from data. With this idea, we propose to estimate $P(C|U,I,M)$ from data, and comparing user interest for different items by Natural Direct Effect (NDE), which compare the causal effect condition on same whatever $C$. According, \cite{hanwang_longtail}, NDE can be approximated as following: 
% \begin{equation} \label{eq:nde}
% \begin{split}
%     NDE(C=1|u,i) & = P(C|do(u,i),M=m^* ) - P(C|do(u,i^* ),m=m^* ) \\
%     &= P(C|u,i,m^* ) - P(C|u,i^* ,m^* )
% \end{split}
% \end{equation}
% , where $do$ means intervene on the variable, and $i^*$ and $m^*$ is dummy value. And because we do ranking tasks, we can directly to compare $P(C|u,i,m^* )$ between items for the user $u$.

% Our goal to estimate the correlation caused by $I \rightarrow C$ which represents the clicking caused by user-item matching. But previous CF models directly estimate $P(C|U,I)$, means that it will mislead by the other two correlations. The better way is to estimate P(C|U,I,M) with the following reasons: (1) $M$ is observable. (2) This term is not influenced by the confounder. (3)According to \cite{pearl_primer}, Natural Direct Effect (NDE), which compare the causal effect condition on same $Z$, can be used to realize our goal.  And according to \cite{pearl_primer,hanwang_longtail}, NDE can be computed as following for our graph:
% \begin{equation} \label{eq:nde}
% \begin{split}
%     NDE(C=1|u,i) & = P(C|do(u,i),M=m^* ) - P(C|do(u,i^* ),m=m^* ) \\
%     &= P(C|u,i,m^* ) - P(C|u,i,m^* )
% \end{split}
% \end{equation}
% , where $do$ means intervene on the variable, and $i^*$ and $m^*$ is dummy value. And because we do ranking tasks, we can directly to compare $P(C|u,i,m^* )$ between items for the user $u$.




% \subsection{Method}
% Based on above analyses, we proposed our method in figure~\ref{fig:framework}. As showing in figure, it has different flows for training and inference. In the following, we will first introduce our model. Then we introduce the training and inference paradigm.

% \subsubsection{Model.} In our model, we aim at estimating the $f_C(U,I,M)$  (or the $P(C|U,I,M)$), so it should take three inputs $u,i$, and $m$. As bottle block that shown in figure~\cite{fig:frame}, We first input the $(u,i)$ to an basic recommendation model that can compute the user-item matching, such as MF. Then we get:
% \begin{equation} \label{eq:base-rec}
%     k_ui = f_{\Theta} (u,i)
% \end{equation}
% where $f_{\Theta}$ represent basic recommendation model and $\Theta$ is corresponding model parameters, and $k_ui $ the output. Then we model $f_C(U,I,M)$ as following:
% \begin{equation} \label{eq:f_c}
%     f_C(u,i,m) = \alpha(k_{ui}) \times m^{'\gamma}  
% \end{equation}
% where 
% $$ m^{'} = \frac{m -  m_{min} }{ m_{max} - m_{min} } $$
% to re-scale $z$ to $[0,1]$, and the $m_{min}$ and $m_{max}$ are the maximum and minimize of the input $m$, the reason will be introduced in later. '$\times$' represents product, and $\gamma$ is a hyper-parameter. $\alpha$ is an activation function to transfer the value space of $k_ui$ to one desired space. We take the form that the product of user-item matching and popularity to represent that popularity directly affect interaction by increasing the user-item matching of which the items are more popular. Note that the increasing does not refer to the absolutely increasing values, but it has increased than unpopularity one. The design is fit to the conformity,\ie users tend to follow the majority to consume popular items. So the function of the $\gamma$ is to control the degree of influence of popularity. And it worth to note that the value space of $k_{ui}$ is depend on the basic recommendation model, it values can be both positive and negative, we can't directly multiply it with the popularity, because there is one inconsistent phenomenon that one positive value times a value in $(0,1)$, the results will be smaller than the positive values, but one negative value times the same value, the result will be greater than the negative value, this means that that times a same value has opposite effects for positive and negative values. $\alpha(\cdot)$ is used to make transfer $k_ui )$ always be positive, the function that we use is defined as following:
% \begin{equation} \label{eq:alph-function}
% 	\alpha(x) = \begin{cases}
% 	e^{x}, &\text{if } x \leq 0 \\ %\mathbb{Q}\\%mathbb花体字符
% 	x + 1, &\text{else}  %\in \mathbb{R}\setminus\mathbb{Q}	
% 		   \end{cases}%\text是为了在数学公式中处理中文
% \end{equation}
% The function is similar to elu~\cite{elu} but be always great than 0. Our model is very sample, but the key operation that explicitly control the the item popularity in the model,\ie taking popularity as an input, is key very important and essential, without it, the model will be mislead.    

% \subsubsection{Training.}  
% At first. Different with previous work that take the global popularity of data to be considered. We think that we should use local popularity for the different stages. The reasons are following: (1) From the datat generated processing, the dataset is not generated at a time, it means that the interaction happens in different environments, such as item popularity will change with time going by as showing in figure~\ref{fig:drit_showing}. The instances of $M,Z$ is not same for the interactions that happens in different time. (2) Our goal is fit the $f_C(u,i,M)$ on $M$ for each $(u,i)$ pair, if the global popularity is taken, there is only one sample on $f_C(u,i,M)$, it's hard to learn it well. It's better to know the popularity when the interaction happening, but it's hard to get this information. So we take compute popularity of different stage as an approximation. If there is know information about stage information, artificial division is also selectable. Assume that we have $T$ stages of data $\mathcal{D}=\{\mathcal{D}_1,\dots,\mathcal{D}_T \}$. for each interaction $(u,i)$ on $\mathcal{D}_t$, compute its corresponding $M$ as \ref{eq:pop_define} on dataset $D_t$, as denote it as $m^t$, and then form a instance $(u,i,m^t)$ for $U,I,M$. Please note $m^t$ only refer to different instance of $M$ at different stage. When training, the training samples are randomly selected from the total sets without distinguishing the stage. 

% At last, we formulate the loss as:
% \begin{equation} \label{eq:loss}
%     L(B) = L_{0} (\Theta|B) + \lambda \| \Theta \|
% \end{equation}
% where the $B$ represent a batch of data, and $\Theta$ represents the model parameters, $\lambda$ is regularization hyper-parameter, and the $L_0$ represent recommendation loss, such as BPR loss in equation~\ref{eq:bpr}. Another thing that should note be noticed is that the output of $f_C$ may need to be inputed into an function to make it suitable for the $L_0$. Such as, for Binary Cross Entropy loss, if the $f_C$ is in $(0,+\infty)$, $\frac{x}{x+1}$ can be a suitable function. 

% At last, we summarize our training processing in Algorithm \ref{alg:PD-learing}. line 1 refer to split dataset if need. line 2-4 refer to compute $M$ on different stage, and 5-9 is the training process. One the last thing that should be noticed is that $z_min$ and $z_max$ refer to the maximum and minimum for different stages, to make the popularity at different comparable. 

% \begin{algorithm}[t]
% 	\caption{PD-learning}
% 	\LinesNumbered
% 	\label{alg:PD-learing}
% 	\KwIn{Dataset D, number of stage T }
% % 	\KwOut{Updated recommender $W_{t+1}$}
%     \If{ $\mathcal{D}$ don't have stage}{split D to T stage \{$\mathcal{D}_1 ,\dots,\mathcal{D}_{T}$\} along time \;}
% 	\For{t $\in {1,...,T}$}{ $\forall (u,i)$, computing its popularity  $m^t$ on $D_t$ by \eqref{eq:pop_define} } 
% % 	Match each interaction $(u,i,t)$ with $z^t$\;
% 	\While{Stop condition is not reached}{
% 	randomly sample one batch interactions B in D\;
% 	Compting $f_C(u,i,m^{t} )$\;
% 	Update $\Theta$ by optimization $L(B)$. 
% 	}
% \end{algorithm}

% \subsubsection{Inference}. For inference, there are two ways to do recommendation. The first the NDE, and the other is to inject some desired popularity bias by interven on $M$. Recall the NDE introduced in Eq.\eqref{eq:nde}, for recommendation:
% \begin{equation}
% \begin{split}
%   NDE(C|u,i) & = f(C|u,i, m^* ) - f(C|u,i^* , m^*) \\
%     & = \alpha(k_ui ) (m^* )^\gamma - \alpha(k_{ui^\star}) (m^* )^\gamma \\
%     & = \alpha(k_ui) Q_1 - Q(u)
% \end{split}
% \end{equation}
% where $m^\star$ and $m^\star$ is dummy values, $Q_1$ is a constant, and Q(u) is only related to one user. It's obviously that we can ranking user based on $k_{ui} $ directly. This recommendation is similar to one ideal state if let all the items has popularity, which items is better to be recommended to users.  

% The other recommendation is to consider inject desired popularity bias to recommendation list or getting better recommendation accuracy with some extra popularity bias, such as recommend more item that will be popular in the near future if we can predict it. To this goal, we take $P(Y|do(U=u,U=i,M=\hat{m}_i ))$ to recommend items with desired popularity, where the $\hat{m}_i$ is the predicted popularity. According to \cite{pearl_primer}, for our graph, we have:
% \begin{equation}
%     P(C|do(U=u,I=i,M=\hat{m}_{i} )) = P(Y|u,i,\hat{m}_{i})
% \end{equation}
% so, we recommend items to users with desired popularity by:
% \begin{equation}
%     f_C(u,i,\hat{m}_i) = \alpha(k_ui ) (\hat{m}_i)^\gamma
% \end{equation}
% In this work, we take to two methods to predict the popularity for testing stage: 
% \begin{itemize}
%     \item[(a)] $\hat{m}_{i} = m_{i}^{T}$
%     \item[(b)] $\hat{m}_{i} = m_{i}^{T} + \alpha (m_{i}^{T} - m_{i}^{T-1})$
% \end{itemize}
% where the $\alpha$ is a hyper-parameter. We take (a) with the observation in Figure~\ref{fig:drit_showing} that the more near the two stages are the more similar popularity they have. (b) is based on (a), but considers the trend of popularity drift, which is usually helpful for time series prediction. In this work, we don't focus on how to predict popularity better, we don't develop other approaches.




% The better selection is that treat the interactions of one item has different popularity in different time period. But we don't know how many times recommendation happens in data. So take a approximation: at first, we split dataset to $T$ chunks along timestamp, where each chunk represent a time periods. then, we compute the distribution of popularity denoted as $z^{t}$ for each period $t$.  Third, matching each interaction $(u,i)$ a corresponding popularity $z^t$ to get $(u,i,z^{t})$. At last, $(u,i,z^{t})$ is a training sample for $P(C|U,I,Z)$. In this way, we have also increased the counts of instances of $P(C|u,i,Z)$ on $Z$ to make it can be learned better. At last, we summary the learning program in Algorithm \ref{alg:PD-learing}.



% $Z=[1,0]: 0.6 Z=[0,1] 0.4$, item1 and item2, 10 times recommendation, each time 10 recommendation. if items correspoding values in Z, then it is has be recommend 8 times to be recommend.
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c}
%         Z     &  item 1  &  item 2\\
%         $Z_1$ &  48 (36 m = 1 )      &   12(3 m=0) \\
%         $Z_2$ &  8  (2  m = 0 )      &    32 (24 m = 1)
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}


% \subsubsection{Confounder}
% In causation, confounder is defined as following~\cite{pearl2009causality}:If a variable is a common cause of two other variables, then variable is called a confounder of the other two variables. such as in our graph $Z$ is the confounder of $M$ and $I$ in our graph, and also the confounder of $I$ and $C$.

% \subsubsection{Intervention.} Intervention on some variable $I$ refers to change the value of the variable to the desired one by force. "by force" means that cut down the edge arrow into the variable, or de-correlate the variable with its fathers. Usually intervention experiments are used to estimate causal effects of the treatmeant $I=i$ to the target $C$, denote as $P(C|do(I))$. It's worth noted that cutting down one path will not influence the mechanisms represented by other edges, such as cutting down $Z\rightarrow I$ will not influence $P(C|U,I,M)$. 


% \subsubsection{Correlation is not causation}
% Usually, people subconsciously treat correlation as causation, such as taking $P(C|U,I)$ as the causal effect of $(U,I)$ to $C$. In some case, the correlation is same to causality. But correlation is not causation~\cite{pearl2009causality}. One most known case is that when a causal graph contain a confounder between two nodes, then the two nodes will exhibit some spurious correlation which not caused by their causal relation. But current mechian learning methods is used to capture correlation without distinguishing the spurious and true correlation caused by causality. Let's show this by a example:  

% Assuming that there one user that interacts with two items --- item1 and item 2. $Z$ is a two dimensions distribution, and its space is $\mathbb{[0,1],[1,0]}$, the higher values in one diemension represent that this dimension corresponding item is more popular and has higher probability to be recommended more. Assume that the user has the same interaction probability $1/2$ to interacted with both the items. And if a item is popular that the other, its interaction will increase $1/4$ and the other one will decrease $1/4$. Then we gernert the data as table
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c|c}
%          & Z & item1 & item2\\
%          & $z_1$ & 
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}


% Aussume that $U_X,U_Y,E_Y$ are independent standard Gaussian distributions in the figure~\ref{fig:example} , the question is that how many $Y$ will increase if $X$ increase one unit without other conditions changed. The answer is $b$ obviously. But If we don't know all the functions in figure~\ref{fig:example},  we may directly regress Y on X:
% $$Y =  d X + e$$
% Then we have $d = \frac{E(XY)}{var(X)} = \frac{b(a^2 + 1)+ca}{a^2 +1} $, the the answer is $d$. The effect from $X$ to $Y$ will be under- or over-estimated. 
% It's wrong to esitmate the really causal effect from $X$ to $Y$ by $P(Y|X)$ when there exist a confounder $A$ of $X$ and $Y$. For our graph in figure~\ref{fig:rec_causal_pre_now}(b), we can't directly to estimate the $P(C|U,I)$ to represent users and items matching. 

% \subsubsection{Backdoor Adjusting}
% Usually, If we want to estimate the truely effect on $Y$ caused by $X$, intervention experiments(RCTs) are the directly selection, but in most case that it's not  practical to conduct RCTs. Is there any way to realize this goal directly on observed data? Fortunately, \cite{pearl2009causality} has introduce a method called  Back-Door Adjustment can relize this by adjusting the causal graph to get a adjusted probability expression. It has three considerations: (1) block all spurious paths between X and Y (back-door path, such as $X\leftarrow A\rightarrow Y$) (2) leave all directed paths from X to Y unperturbed, and (3)create no new spurious paths.  




% \subsection{Better User-Item Matching}
% For recommendation, we have introduced the causal graph with popularity in section~\ref{sec:intro}, shown in figure \ref{fig:rec_causal_pre_now} (b). We would 
% emphasize that the Z does refer to the distribution of all items popularity instead of one item popularity, i.e recommender systems take all items' popularity to consider and decide to recommend which items more. In a word, high popularity is a relative term. %Some readers may think that there also a edge $I \rightarrow Z$, note that we assume that the function of each edge is fix. But the popularity of one item will change with time going by, so we can't add this path. What'more we can think this path has added into $I\right arrow directly$   

% Because popularity $Z$ is a confounder, estimating user-item matching by $P(C|U,I)$ can't reflect the true matching. It is better to model $P(C|do(U,I))$ to estimated the true matching. Applying Back-Door Adjustment,
% we get:
% \begin{equation} \label{eq:backdoor-pop-bias}
%     P(C|do(U,I)) = \sum_Z P(C|U,I,Z)P(Z)
% \end{equation}

% The following is the derivation process: According Back-Door Adjustment, compute P(C|do(U,I)) of the left graph is equal to compute $P_r(C| U,I)$ (where r represent right) of the right graph that cut down the path $Z\rightarrow I$ in figure~\ref{fig:rec_causal_pre_now} (b), we have: 
% \begin{equation}
% 	\begin{split}
% 	P(C|do(U,I)) & \overset{(1)}{=}  P_{r} (C|U,I)\\
% 	& \overset{(2)}{=} \sum_Z P_{r}(C|U,I,Z)P_{r}(Z|U,I)\\
% 	& \overset{(3)}{=} \sum_Z P_{r}(C|U,I,Z)P_{r}(Z)\\
% 	& \overset{(4)}{=} \sum_Z P(C|U,I,Z) P(Z)
% 	\end{split}
% \end{equation}

% where (1) is because of Back-Door Adjustment, (2) is because of Bayes' theorem, (3) is because of that $U,I$ are independent with $Z$ in the right graph, and for (4), $P(C|U,I,Z) = P_{r}(C|U,I,Z)$ means that causal mechanism that $(U,I,Z)$ cause $C$ will note changed with the cutting down operation. $P(Z) = P_{r}(Z)$ represent $Z$ has the same distribution in the two graphs. 

% Obviously, $P(C|do(U,I))$ is different with: 
% \begin{equation} \label{eq:bayes-pop-bias}
%   P(C|U,I) = \sum_Z P(C|U,I,Z)P(Z|U,I)
% \end{equation}.
% It's easy find the differences are P(Z|U,I) and P(Z) for Eq.\eqref{eq:bayes-pop-bias} and Eq.\eqref{eq:backdoor-pop-bias}. P(Z) instead of P(Z|U,I) means that $Z$ is independent with $U$ and $I$, this is the key spirit of intervention experiments by cutting down $Z\rightarrowI$. This is also the key point that Back-Door Adjustment can realize the same goal to intervention experiments directly from observed data.  

% But Backdoor Criterion tell us we can directly estimate $P(Y|do(U,I))$ from observation data with overlapping assumptions\cite{overlapping}.
% \subsection{Popularity-bias Deconfounding}
% % \subsubsection{Estimate Causal Effect}

% As discussing above, popularity brings confounding effect, we should estimate the causal effect $P(C|do(U,I))$ instead of the correlation $P(C|U,I)$ to represent user-item matching. In this way, we can remove the confounding effect. To estimate $P(C|do(U,I))$, according its probability expression in Eq.\eqref{eq:backdoor-pop-bias} and previous work~\cite{wang2019blessings}, it can be directly estimated by the two steps: 1) estimating $P(C|U,I,Z)$ from data. 2) computing the final $P(C|do(U,I))$ based on the $P(C|U,I,Z)$ and $P(Z)$. Next, we will implement the two steps in a learning perspective.

% \noindent \textbf{Step 1. Estimating  $P(C|U=u,I=i,Z=z)$.} To make our model can be applied to different models, We use a function $h(u,i,z)$ to represent it but not restrict its values always in $[0,1]$. The $h(u,i,z)$ has following form:
% \begin{equation} \label{eq:do-matching}
%     h(u,i,z) = \alpha(k_{ui}) \times \hat{z}_{i}^{\gamma}  
% \end{equation}
% where 
% $$ \hat{z} = \frac{z_i -  z_{min} }{ z_{max} - z_{min} } $$
% means that the  $z_i$ corresponding to item $i$, is re-scaled to $[0,1]$; $k_{ui}$ is the output of base model to represent user-item matching, assuming that it can be inputted into an activate function $\alpha(\cdot)$ to make the result $\alpha(k_{ui})$ be in $(0, \infty) $. We take the form $\alpha(k_{ui}) \times \hat{z}^{\gamma}$ to represent that popularity directly affect interaction by increasing the user-item matching of which the items are more popular. (Note that the increasing refer to relative increasing instead of absolutely increasing values). The design is fit to the conformity,\ie users tend to follow the majority to consume popular items. And we activate $k_{u,i}$ to $(0,\infty)$ based on the following consideration: there is one inconsistent phenomenon that one positive value times a value in (0,1), the results will be smaller than the positive values, but one negative value times the same value, the result will be greater than the negative value, this means that that times a same value has opposite effects for positive and negative values. $\gamma$ is a hyper-parameter to control the degree of the influence of popularity.  Assuming that $k_{ui}\in(-\infty,\infty)$, we provides the following activating functions:
% \begin{equation} \label{eq:alph-example}
% 	\alpha(x) = \begin{cases}
% 	e^{x}, &\text{if } x \leq 0 \\ %\mathbb{Q}\\%mathbb花体字符
% 	x + 1, &\text{else}  %\in \mathbb{R}\setminus\mathbb{Q}	
% 		   \end{cases}%\text是为了在数学公式中处理中文
% \end{equation}
% Then, The output of $h(u,i,z)$ can be input another activation function $\beta(\cdot)$ to  re-scale  it for loss:
% \begin{equation}\label{eq:do-re-scale}
%     f(u,i,z) = \beta(h(u,i,z))
% \end{equation}
% At last, we take the following loss:
% \begin{equation} \label{eq:loss}
%     L(B) = L_{0} (\Theta|B) + \lambda \| \Theta \|
% \end{equation}
% Where $L_{0}(\theta|D)$ denotes one recommendation loss,such as the widely  used bpr-loss~\cite{bpr-loss} and log-loss~\cite{log-loss}, the $\Theta$ is the all parameters for the model, and $B$ represent one batch data. Note that Utilizing which activation function $\beta(\cdot)$ in equation~\ref{eq:do-re-scale} depend on which $L_0$ is taken. Such as, when $L_0$ is bpr loss, the following $$ \beta_{1}(x) = x \in [0,\infty)  \, where\, x\gep 0$$ is suitable. When $L_0$ is log-loss, the following
% $$ \beta_{2}(x) = \frac{x}{x+1} \in [0,1) , where x \geq 0 $$
% can be used to make the outputs to represent probability.

% At last, we need optimize the model. How to generate samples is very import. Note that the dataset is not generated at a time, it means that the interaction happens in different environments, such as item popularity will change with time going by as showing in figure~\ref{fig:drit_showing}. So the instance of confounder $Z$ is not same for the interactions that happens in different time. The better selection is that treat the interactions of one item has different popularity in different time period. But we don't know how many times recommendation happens in data. So take a approximation: at first, we split dataset to $T$ chunks along timestamp, where each chunk represent a time periods. then, we compute the distribution of popularity denoted as $z^{t}$ for each period $t$.  Third, matching each interaction $(u,i)$ a corresponding popularity $z^t$ to get $(u,i,z^{t})$. At last, $(u,i,z^{t})$ is a training sample for $P(C|U,I,Z)$. In this way, we have also increased the counts of instances of $P(C|u,i,Z)$ on $Z$ to make it can be learned better. At last, we summary the learning program in Algorithm \ref{alg:PD-learing}.

% \begin{algorithm}[t]
% 	\caption{PD-learning}
% 	\LinesNumbered
% 	\label{alg:PD-learing}
% 	\KwIn{Dataset D, the number of split chunks T }
% % 	\KwOut{Updated recommender $W_{t+1}$}
% 	Split D to T chunks \{$D_1,\dots,D_{T-1}$\} along time \;
% 	Compute each chunk popularity $z^t$ by equation \ref{eq:pop} \;
% 	Match each interaction $(u,i,t)$ with $z^t$\;
% 	\While{Stop condition is not reached}{
% 	randomly sample one batch interactions B in D\;
% 	Update $\theta$ by optimization $L(B)$. 
% 	}
% \end{algorithm}





% \noindent \textbf{Step 2. Estimating  $P(C|do(U,I))$.}
% To simplify, we using the the following equation to represent $P(C|do(U=u,I=i))$ with $g(u,i)$ using the $h(u,i,z)$ in the step 1:
% \begin{equation}
% \begin{split}
%     g(u,i) & =\sum_z h(u,i,z)p(z) \\
%     & = \sum_z \alpha(k_{ui}) \sum_z\hat{z}_i^{\gamma}p(z) \\
%     & = \alpha (k_{ui}) E_Z(\hat{Z}_{i}^{\gamma})
% \end{split}
% \end{equation}
% where $E(\hat{z}_{i}^{\gamma}) = \sum_z\hat{z}_i^{\gamma}p(z)$. There are two way to compute it:
% \begin{itemize}
%     \item[(a).] empirical estimation:
%     $$E(\hat{Z}_{i}^{\gamma}) = \frac{1}{T} \sum_t \hat{z}_{i}^{t\gamma} $$
%     \item[(b).] ideal assumption:
%     $$ E(\hat{Z}_{i}^\gamma ) = E(\hat{Z}_{j}^\gamma ) = constant $$
% \end{itemize}
% It's obvious that (a) is a directly way to estimate $E(\hat{z}_i)$, it means that we take t-th period popularity $z^{t}$ as an instance of $Z$, and then the mean of instances is taken as expectation. But it is not a good estimation, since the following reasons: (1) we only have few instances of $Z$, the post-distribution may be very different with the truly $P(Z)$. (2) If we need to recommend items for future, what the future distribution of $Z$ may be far away the post distribution of $Z$ on the dataset. (3) If $P(Z)$ is changed, the result of $P(Y|do(U,I))$ will also be changed, so empirical estimation can't represent a generalized result. To cope with these problems, following \cite{hanwang_uniform}, we think that assuming $P(Z)$ is a uniform distribution on it the total space, can be a suitable choice, if we has not any information regrading what the $P(Z)$ will be. Taking this assumption, then the expectation of each dimension $z_i$ will be the same. It result in the method (b). We will compare the two methods in the experiments, but take the (b) as the default setting. 

% Combine step (1) with (2), it results in our Popularity-bias Deconfounding (PD) method. 

% %  \subsection{Inference with drifted popularity}
%  \subsection{Popularity-bias Adjusting}
%  Considering the need of introducing desired bias into the system, such as promoting the items that have the potential to be popular, the core is equal to adjust the popularity be the same to the desired one $z$ by force. To realize this goal, we can intervene $Z=z $ and then we can intervene $U=u$ and $I=i$ to simulate the responses,\ie $P(C|do(U=u,I=i),do(Z=z )$. Then we can recommend item with the responses to do real recommendation to get higher recommendation accuracy. To compute the  $P(C|do(U=u,I=i),do(Z=z )$, we only need to cut down the paths that arrow into $Z$ of the right graph in figure~\ref{fig:rec_causal_pre_now}. There are not any these types of paths. So we can compute it still on the right graph, we can get:
%  \begin{equation}
%  P(C|do(U=u,I=i),do(Z=z ) = P(C|u,i,z ) 
%  \end{equation}
%  Then, we can use the $h(u,i,z)$ in PD to compute the values and recommend items. We name this method as PDA.
 
% %  If we can predict what the popularity will drift towards. Assume that the function $f(\cdot)$ will not change with time going. We can predict more accurately predict by counterfactual inference:
% %  $$ E(C|do(U=u,I=i),do(Z=z_{pre}) = E(C|u,i,z_{pre})  = f(u,i,z_{pre})$$
% %  where $z_{pre}$ can be predicted by any method. In this paper, we take the popularity of the most recent period data, and a linear predicted popularity as predicted popularity.  
 
 
 
%  \subsubsection{Instantiation on Matrix Factorization}
 
%  To demonstrate how our proposed PDA framework works, we provide an implementation based on \textit{Matrix Factorization} (MF), which is a representative embedding model for recommendation. Given a user-item pair $(u,t,m^t)$, where $t$ represent interaction in stage t and $m^t$ is corresponding popularity, MF predicts the user-item matching as
%  \begin{equation}\label{eq:mf}
%      k_{ui} = p_{u}^{\top} q_{i}
%  \end{equation}
%  where $p_{u} \in \mathbb{R}^d$ and $p_{u} \in \mathbb{R}^{d}$ represent the the embedding of $U=u$ and $I=i$ respectively, and $d$ is the embedding size. We take the $\alpha(\cdot)$ in equation \eqref{eq:alph-example} and $\beta_{1}$ as the activation functions for equations \eqref{eq:do-matching} and \eqref{eq:do-re-scale} to get:
%  $$ f(u, i, m^t ) = \alpha(k_{ui})\times \hat{m}_{i}^{t} $$.

% For recommendation Loss $L_0$, we adopt BPR loss in equation~\ref{eq:bpr}, which is common choice for recommendation. For each 
% $(u,i,m^t)$, we randomly sample 1 unobserved
% interaction of u, denotes its item as $i^{-}$, to represent negative interaction, and regarding its $M$, we directly make it same to the $m^t$ of the positive one. Then BPR loss in equation \eqref{eq:bpr} has been used.
% \begin{equation}
%     L_{0} (P,Q|D) = \sum_{(u,i,i^{-},m^{t})\in D} log(\sigma(f(u,i,m^t ) - f(u,i^{-}, m^t))) 
% \end{equation}
% where $P,Q$ denote the embeddings of all users and items, and $\sigma(\cdot)$ is the sigmoid function.





% For the recommendation loss L0, we adopt the pointwise log
% loss, which is a common choice for recommender training [15, 26].
% For each interaction (u,i) ∈ Dt
% , we randomly sample 1 unobserved
% interactions of u to form the negative data set D
% −
% t
% . Then the log
% loss is formulated asFor the recommendation loss L0, we adopt the pointwise log
% loss, which is a common choice for recommender training [15, 26].
% For each interaction (u,i) ∈ Dt
% , we randomly sample 1 unobserved
% interactions of u to form the negative data set D
% −
% t
% . Then the log
% loss is formulated as
% \begin{algorithm}[t]
% 	\caption{PD/PDA}
% 	\LinesNumbered
% 	\label{alg:PD-PDA}
% 	\KwIn{Dataset $\mathcal{D}=\{(u,i,m_{i}^{t})\}$, model:PD or PDA}
% 	\While{stop condition is not reached}{
% 	Update model parameters $\Theta$ by optimizing Equation~\eqref{eq:bpr}\; 
% 	if PD, validate model with $ELU^{'}(f_\Theta (u,i))$\;
% 	if PDA, validate model with Equation~\eqref{eq:mf}\;
% 	}
% % 	// Step 2: inference with $P(C|do(U,I))$ \;
%     // testing\;
%     if PD, recommend items using $ELU^{'}(f_\Theta (u,i))$\;
% 	if PDA, Recommend items using Equation~\eqref{eq:mf} for PDA\;%(or $ELU^{'}(f_\Theta (u,i))$ for PD)\;
% \end{algorithm}

\begin{algorithm}[t]
	\caption{PD/PDA}
	\LinesNumbered
	\label{alg:PD-PDA}
	\KwIn{dataset $\mathcal{D}=\{(u,i,m_{i}^{t})\}$; hyper-parameter $\gamma$; predicted popularity $\{\Tilde{m}_i\}$; \textit{mode}: PD or PDA }
	\While{stop condition is not reached}{
	Update model parameters $\Theta$ by optimizing Equation~\eqref{eq:bpr}\;
	\lIf{mode==PD}{validate model with $ELU^{'}(f_\Theta (u,i))$}
	\lElse{validate model with Equation~\eqref{eq:mf} (simplify $\Tilde{\gamma}=\gamma$)}
% 	\If{PD}{validate model with $ELU^{'}(f_\Theta (u,i))$\;}
% 	\Else{validate model with Equation~\eqref{eq:mf}\;}
% 	\ifthenelse{PD}{A}{B}
	}
% 	// Step 2: inference with $P(C|do(U,I))$ \;
    % // testing\;
    \lIf{mode==PD}{recommend items using $ELU^{'}(f_\Theta (u,i))$}
    \lElse{recommend items using Equation~\eqref{eq:mf} (simplify $\Tilde{\gamma}=\gamma$)}
\end{algorithm}
 



